Large Scale Question Answering using Tourism Data

We introduce the novel task of answering entity-seeking recommendation questions using a collection of reviews that describe candidate answer entities. We harvest a QA dataset that contains 47,124 paragraph-sized real user questions from travelers seeking recommendations for hotels, attractions and restaurants. Each question can have thousands of candidate answers to choose from and each candidate is associated with a collection of unstructured reviews. This dataset is especially challenging because commonly used neural architectures for reasoning and QA are prohibitively expensive for a task of this scale. As a solution, we design a scalable cluster-select-rerank approach. It first clusters text for each entity to identify exemplar sentences describing an entity. It then uses a scalable neural information retrieval (IR) module to select a set of potential entities from the large candidate set. A reranker uses a deeper attention-based architecture to pick the best answers from the selected entities. This strategy performs better than a pure IR or a pure attention-based reasoning approach yielding nearly 25% relative improvement in Accuracy@3 over both approaches.

==> experiments.tex <==

\section{Experiments}\label{sec:experiments}

We ask the following questions in our experiments: (1) Is constructing the representative document using clustering better than other sentence selection baselines? (2) To what extent are non-neural baselines such as TF-IDF retrieval, effective for this task? Could they be useful in pruning the search space for a downstream module with deeper reasoning and re-ranking? %(2) How well does QESE perform on the full-ranking task?  %(2) In our Question-Entity Siamese (QESE) network, are generating question-dependent entity embeddings helpful? 
%(3) Is constructing the representative document using clustering better than other sentence selection baselines?  %(4) How can the quality of negative samples used in our training be improved? 
%(4) How do state-of-the art neural IR models designed for adhoc-retrieval tasks perform on our task? % for our task?

\subsection{Metrics}

For a question $q$, let the set of top ranked $N$ entities returned by the system be $E_N$, and let the correct (gold) answer entities for the question be denoted by set $G$, then   $Acc@N = \mathbbm{1} ((E_N \cap G)\neq \phi)$, 
%\begin{equation}
 %   ACC@N = \mathbbm{1} (G \in E_N)  
%\end{equation}
where $\mathbbm{1}$\{\} is the indicator function. We report $Acc@3$, $Acc@5$ and $Acc@30$ scores. 

%Note that our metric 
%the highest rank the gold answer ranks is used compute eas ranking correct answer.

\noindent {\bf Mean Reciprocal Rank (MRR): } % For each question we use the highest ranked gold entity to compute MRR.  %Let the set of questions be $Q$, and let $E$ be the ranked list of entities $E$ for a guestion $q$ and $R'_q$ be the list of ranks of the gold entities for the question $q$. Then we define the MRR metric as 
% For a given ranked list of entities $E$, %it is the average of the inverse ranks of each correct answer entity.
% if the entity at rank $r$ is the gold answer entity then the mean reciprocal rank is given by $ $$MRR = \frac{1}{|Q|}\sum_i^{|E|} \frac{1}{r_i}$$.
Let $Q$ be the set of questions in our test set and let $r_i$ be the rank of the highest ranked gold entity for question $q_i \in Q$. The mean reciprocal rank (MRR) is then defined as: $\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$.
%\begin{equation}
%$\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$
%\end{equation}
Note that in case of questions with multiple gold entity answers, both metrics use the gold entity with the highest rank.

\subsection{Hyper-parameter Settings}
All models were trained for 5 days (approx. 14 epochs \footnote{Trained on $6$ K80 GPUs.} for QESE based models) using $10$ negative samples for each QA pair. We used $3$-layer $128$-dimensional bidirectional GRUs to encode questions and review sentences. Input word embeddings were updated during training and USE embeddings returned $512$ dimension embeddings. For all experiments we set $\delta=1$ in our max-margin criterion. We used Adam Optimizer \cite{Adam} with a learning rate of $0.001$ for training. Training the QESE model  took $11.5$ hours per epoch on 4 K-80 GPUs.% and loss stabilization as stopping criteria.


 \begin{table}[]
\scriptsize
\begin{tabular}{c||l|l|l|l}
\textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA layer\end{tabular}} &  16.60              & 22.6                & 51.7                                  & 0.154             \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ Random Sent. \end{tabular}} & 9.64              &      13.79       &                       37.18           &  0.098            \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ BM25 Sent. \end{tabular}} &                 &                &                                  &              \\ \hline


%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Effectiveness of representative documents (Full-ranking task)} \label{tab:ablation}
\vspace*{-2ex}
\end{table}

\subsection{Representative Documents}
%We study if our modeling choice of generating question dependent entity embeddings using the QEA layer was useful. In addition,
We investigate whether document representations created using sentence clusters perform better than randomly selecting $100$ sentences from an entity. As can be seen from Table \ref{tab:ablation} the use of representative sentences result in marked improvement in performance on the full-ranking task. We also tried to create document representations by selecting $100$ sentences from an entity document by indexing them in Lucene and then using the question as a query. We found that this method, understandably, returned very few sentences -- the questions (query) is longer than a sentence on average and the lexical gap is too big to overcome with simple expansion techniques. 


\subsection{Telescoping} \label{sec:baselines}
We compare the following telescoping methods:
%We consider the following non-neural models:
%To demonstrate the challenging nature of the task, we present results from baseline systems using BM25 retrieval baselines as well as a few neural retrieval models.
 
 %To make the task simpler, all methods below only consider candidates that are of the same type as the gold answer and not all possible candidate entities. 
%\subsection{Non-Neural Baselines}
\noindent{\bf Random Entity Baseline:} Returns a random ranking of the candidate entity space.% (of the same type as the gold entity).

\noindent{\bf Ratings Baseline:} Returns a ranking of the candidate entities based on user review-ratings.

\noindent{\bf BM25 Retrieval:} We index each entity along with its reviews into Lucene\footnote{http://lucene.apache.org/}. Each question is transformed into a query using the default query parser that removes stop words and creates a disjunctive term query. Entities are scored and ranked using BM25 ranking \cite{BM25}. Note that this baseline is considered a strong baseline for information retrieval (IR) and is, in general, better than most neural IR models \cite{BM25Good}.  % \cite{BM25} and returned as answers to the question.
% \subsection{Neural Models}
% Since we formulate the task as a ranking problem, we train the model to score a correct answer higher than an incorrect answer \cite{Siamese1,Siamese2}. Specifically, given an entity document ($d_e$) and a question $q$, we generate a score $s_e$ for the entity with respect to $q$ by computing a weighted dot product $s_e$=$qWd_{e}$ and would like $s_p$ $>$ $s_n$ for a correct entity $p$ and an incorrect entity $n$. % All the networks are trained by sampling $10$ negative (incorrect answer) entities for each question-answer pair and using hinge loss 
% This is easily specified to the model by using hinge loss ($max(0,s_p - s_n + \delta$)) between a correct answer ($s_p$) and negative sample ($s_n$) as the objective function. We set $\delta=1$ in our experiments.  %[ ADD HYPER PARAM DETAILS]

\noindent{\bf Review-AVG Model}
%We experiment with a simple neural baseline. % that uses averaged vector embeddings for sentences to represent each document.
Questions are encoded using a self-attended bi-directional GRU \cite{intra-attention} to generate a question representation.% $\phi$. %The  encoded sentence representations are then used as input to another bi-directional LSTM with self attention to create the final question representation $q$.
%Due to the extremely large nature of entity documents, learning document representations using sequence models becomes prohibitively expensive.
We then use universal sentence embeddings (USE) \cite{USE2018} to pre-compute vector representations for each sentence and use them to create the document representations. %Let $s_{ij}$ be the $j$th sentence vector in $i$th review. Let $w^{k}_{ij}$ be the $k$th word in sentence $s_{ij}$. 
% For an entity $e$, we create its embedding ($d_e$) by first averaging the embeddings of sentences in a review to create a review embedding and then define the entity representation as an average of the review embeddings. Formally, entity embedding $d_e$ is given by:%$\sum_{i}\frac{\sum_js_{ij}/|S_i|}{|N_e|}$
%\noindent{\bf Duet v2:} The Duet v2 model \cite{DUET2} using the representative documents created using clustering.
% \begin{equation}
% \small
%     \vspace{-1ex}
%     %d_e=\sum_{i}\frac{\sum_j (\gamma_{ij}
%     d_e=\sum_{i}\frac{\sum_j
%     s_{ij}/|S_i|}{|N_e|}
%     \vspace{-1ex}
% \end{equation}

% where $|S_i|$ is the number of sentences in review $i$ and $|N_e|$ is the number of reviews in entity $e$. As before, the model is trained using max-margin criterion, but using $d_e$ as the entity embedding.
%[ NOTATION TO BE STANDARDIZED]
%\noindent{Duet V2 Model:} We use the neural IR model, DUET, \cite{DUET} which was recently improved to incorporate inverse document frequencies as well as word vectors \cite{DUET2}.
%\noindent{\bf Duet V2 Model:} We use the neural IR model, Duet v2 \cite{DUET2}, which is an improved version of Duet \cite{DUET}. % incorporate inverse document frequencies as well as word embeddings \cite{DUET2}.



\subsection{Results}
\begin{table}[]
\scriptsize
\begin{tabular}{c||c|c|c|c}
\textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Random\\ Entity\end{tabular}} & 0.35               & 0.48               &    3.98                             &   0.008            \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Ratings\\ \end{tabular}}  &         0.39        & 0.83                &   3.46                           & 0.007          \\ \hline  
\textbf{BM25 }   & 6.78                                           &  9.97               &  30.58              &  0.073                                              \\ \hline %\hline
\textbf{Review-AVG}                                                                 &  {7.97 }              &  {11.91 }              &            {30.9 }     &     {0.084}         \\ \hline
\textbf{Duet v2}   &  {\bf 18.27}               &  {\bf 23.9}               &            {\bf 53.7 }     &     {\bf 0.169 }            \\ \hline

%\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline

%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Performance of different telescoping methods (Full-ranking task).} \label{tab:expts}
\vspace*{-3ex}
\end{table}

As can be seen in Table \ref{tab:expts} we find that baselines such as BM25 retrieval that have been used previously for telescoping are not as effective for this dataset. A neural baseline model, Review-AVG, that uses average sentence embeddings also performs poorly on this task, while the DUET v2 model that uses our representative documents has an Acc@3 of about 18\%. We thus, apply the DUET v2 as our method for telescoping by providing the top-50 candidates returned by DUET v2 for deeper reasoning and re-ranking by QESE. All subsequent experiments described in the paper use $100$ sentences from our representative documents. %electing from highly rated (reviewed) entities as answers is also ineffective.


% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.8]{figs/TourQue_Loss_Plot.jpg}
%   %\vspace*{-2ex}
%   \caption{Figure showing the trends in average loss for the first 15 epochs of training. }
%   \label{fig:loss}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-1ex}
%  \end{figure}  
 
%\subsection{Improving Training with Curriculum Learning}
\begin{figure*}[ht]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.65]{figs/TourQue_CANDIDATE_SPACE-10.jpg}
   %\vspace*{-2ex}
   \caption{Entity class-wise break-up of the number of times (and \%) a correct answer was within the top 10 ranks binned based on the size of candidate search space (X-axis).}
   %\vspace*{-3ex}
   \label{fig:space-study}
 %\end{adjustwidth}
 
 }
%\vspace*{-1ex}
 \end{figure*} 
\noindent{\bf Curriculum Learning:} Max-margin ranking models can be sensitive to the quality of negative samples presented to the model while training. %  Consider, Figure \ref{fig:loss} which shows the variation in loss with number of epochs for the models shown in Table \ref{tab:ablation}.
%As we can see, the average loss per epoch follows a similar trend in all three configurations but they have markedly different accuracy. We hypothesize that this is because our models are presented with negative samples that are easy to distinguish from the gold answer. Thus, the model reports low loss early on without needing to learn effectively.
%\subsubsection{Harder Negative Samples}
Instead of presenting negative samples chosen at random from the candidate space, can we exploit knowledge about entities to give harder samples to the model and help improve its learning? %In a task such as ours, where there are challenges of scale, training faster and better could be useful. 
One method of selecting harder samples would be to use the gold entity and find entities {\em similar} to it in some latent space and then present the closest entities as negative samples.  In neural settings, candidate embedding space serves as a natural choice for the latent space; negative samples could be generated by sampling from a probability distribution fitted over the distances from the answer embedding.

We also experiment with two baseline methods of creating entity embeddings: (i) Using the averaged sentence embeddings of the representative documents (AVG. Emb in \ref{tab:curr-style}) (ii) Doc2Vec \cite{doc2vec}. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. %However, we find that both these embeddings spaces result in a skewed distribution with unhelpful samples, and models using these report poorer performance than sampling at random (Table \ref{tab:curr-style}). %and possibly poorer quality embeddings. 
%This highlights the importance of high quality negative samples for our model.

One could also use task specific embeddings from QESE to model the candidate space, % however, we do not have an obvious method of identifying such negative entities (and embeddings). 
%Using our QESE model directly is also not an option as 
however, running running our trained model on the the test data takes $2.5$\footnote{Using $4$ K-$80$ GPUs} days. Generating question specific candidate embeddings for each instance while training (which is nearly $10$ times larger) is thus infeasible.   %while using methods such as doc2vec were resulting in a highly peaked distribution 
We therefore, decide to generate task specific embeddings using our Question-Entity Siamese model but without the QEA layer that learns question independent entity embeddings. Once a model is trained, embeddings can be generated offline and used to generate a probability distribution (per answer entity) for negative sampling.  

Another source of negative samples can be to use the top-k candidates returned by the telescoping method and serve them as negative samples. DUET v2 is a less complex model is faster to run. We're thus able to execute forward-pass on the complete training dataset to get the top-k samples in a reasonable amount of time. [ QUANTIFY?]%Thus for a given QA pair, we sample the  entities (in the embedding space based on this model) and fit a probability distribution using its distance from the answer entity. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. 
As can be seen in the last row of Table \ref{tab:curr-style}, training QESE with harder negative samples with curriculum learning helps train a better model, faster. Interestingly, the negative samples from Duet v2 cause the model performance to drop significantly in the epoch-limited training-time available. %As figure \ref{fig:tough-sampling} shows, using curriculum learning helps converge to better accuracy faster\footnote{The best accuracy for the regular model occurs after $23$ epochs (not shown in Figure \ref{fig:tough-sampling}).} than regular training.  

\begin{table}[]
\scriptsize
\begin{tabular}{c||c|c|c|c}
\textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157}            \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Doc2Vec Emb. \end{tabular}} &    16.77        & 22.73               &                      53.8          & 0.152             \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ AVG Emb. \end{tabular}} &  16.46            &  22.33             & 52.2                                 &  0.159            \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb. \end{tabular}} &{\bf 17.03}            &  {\bf 23.65}         &            {\bf 54.9}   &     {\bf 0.168}    \\   \\ \hline


%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Curriculum learning (CL) with different entity embedding schemes (Full-ranking task)} \label{tab:curr-style}
\vspace{-2ex}
\end{table}
% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA. layer\end{tabular}} &   68.2           &  77.4            &                          94.8        &  0.58            \\ \hline
% \textbf{QESE}   & {69.2}               &  {78.7}               &            {95.2}     &     {0.6 }             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb \end{tabular}} &       {\bf 71.1}      &    {\bf 79.4}           &                     {\bf  95.4}           &      {\bf 0.61 }       \\ \hline


% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Model performance in a reduced candidate space of $100$ entities} \label{tab:small}
% \vspace{-6ex}
% \end{table}
%\subsection{Ensemble Models}
\begin{table}[]
\scriptsize
\begin{tabular}{c||c|c|c|c}
\textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
\textbf{QESE CL}   &  {17.03}               &  {23.65}               &            {54.9}     &     {0.168  }            \\ \hline
\textbf{Duet v2}   &  {18.27}               &  {23.9}               &            {53.7 }     &     {0.169 }            \\ \hline
\hline
\textbf{\begin{tabular}[|c|]{@{}c@{}}QESE CL\\ + Duet v2 \end{tabular}} &{\bf 19.27}            &  {\bf 25.32 }         &            {\bf 54.9 }   &     {\bf 0.177}   \\ \hline

%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Performance of (i) Duet v2 (ii) Ensemble model with QESE CL + Duet v2} \label{tab:duet}
\end{table}
\noindent{\bf Full Model:} Finally, we evaluate our full model; it uses Duet for pruning the candidate answer space and then QESE CL to re-rank the shortlisted answers. Table \ref{tab: telescope}


\begin{table}[]
\small
\begin{tabular}{l||l|l|l|l}
%\hline
                                                                       & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}l@{}}QESE CL\\ (Task emb.)\end{tabular}} &   23.45             & 34.2               & 81.49                &  0.230            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}QESE CL \\ (Duet)\end{tabular}}     &    40.64            & 53.04               &  91.59               & 0.369        \\ \hline     
\end{tabular}
\caption{QESE CL re-ranking the pruned candidate space returned by Duet. QESE CL with (i) Task specific embeddings for negative sampling (ii) Random Negative sampling from top-50 candidates returned by Duet}
\label{tab:telescope}
\end{table}
\noindent{\bf Duet v.s. QESE (Full Ranking task):} A deeper study using the validation set reveals that both models have different strengths and that at top-3, they correctly answer different sets of questions; between 45-52\% of the questions answered by one model were not answered by the other\footnote{At top-$30$, the percentage of non-overlapping correctly answered questions reduces to 22-25\%.}. Further, we find that Duet v2 which is a shallow reasoner based on matching local and distributed text representations, gains by correctly answering more questions with large candidate spaces. %On other hand, QESE CL, which is a deep reasoner (and thus, slower to train), does not train enough in the same time frame to be as effective in very large search spaces. %Note, however that both models have similar performance when we compare their Acc@5 and Acc@30. %The set of questions answered correctly by both models@30 %Further, about 43\% of the questions answered only by QESE were for hotels and attractions, while for the Duet V2 model it is 27\% -- Duet v2 correctly answers a larger fraction of restaurant questions. 




%We thus, build a simple neural classifier (trained on validation set) that uses the strengths of both models and chooses between the two models for answering. It uses question embeddings from QESE CL along with features to indicate target entity-type and we find that this ensemble model results in improved performance (Table \ref{tab:duet}). 
%To summarize, we find that both, shallow and deep reasoners have different strengths; both models answer  
%[ADD COMMENT ABOUT HOW MULTIPLE MODELS STRENGTHS]

\noindent{\bf Effect of size of candidate space:}
%[TO BE UPDATED]


As mentioned earlier, existing QA tasks operate in a much smaller candidate search spaces. In this section we study the role the size of candidate search space might play on model performance. The plots in Figure \ref{fig:space-study} show the number of times the gold answer was in the top-10 ranks for questions from each entity class\footnote{Recall that each question has its own candidate space}. The results have been binned based on the size of the candidate space ($0-100$,$100-1000$,$1000+$). Questions on restaurants dominate the dataset and also have a larger candidate space with $1553$ questions in the validation set having a search space greater than $1000$ candidates. Of this, only $385-431$ ($25-28$\%) of the questions are answered correctly in the top-10 ranks. In contrast, questions on hotels and attractions largely have a search space of $1000$ candidates or less. Of these, $50$\% of the questions on hotels are answered correctly in the top-10 ranks while the $59$\% of the questions on attractions are answered correctly. 

%To further highlight how the number of candidate answers affect model performance, we also compared the performance of our models with a smaller candidate space of $100$ entities ($1$ correct and $99$ randomly sampled incorrect entities). A comparison between Table \ref{tab:curr-style} \& Table \ref{tab:small} demonstrates that, not only does a large candidate space cause the performance of all models to suffer, it is also likely that only a small percentage of candidate entities are confusing. Thus, we believe that if we had a scalable and effective method of identifying confusing candidate answers for each question, it could help in training, as well as, in enabling a telescope setting for pruning the search space, as used in existing QA tasks \cite{drqa,R3}. % could be helpful in our task. %This also reinforces our belief that while a majority of the candidates are easy to d

%\subsection{Qualitative Study}
% In order to visualize what our model is learning, we study the attention weights applied to tokens in a question and the review sentences. Figure \ref{fig:attention} shows an example from the validation set. Here, the user is looking for recommendations for places to stay and the review sentences shown are for the top ranked (and correct) entity answer (Marina Bay Sands, Singapore) returned by our system. It is interesting to note that the model focuses on descriptive words in reviews while attempting to rank entities. 

% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.3]{figs/Attention_Visualization_1.jpg}
%   % \vspace*{-2ex}
%   \caption{Visualization of attention weights. Darker colours indicate higher attention weights. Review sentences shown  ranked in order of sentence level attentions. Truncated for ease of presentation.}
%   \label{fig:attention}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-2ex}
%  \end{figure}  

\section{Conclusion}
In contrast to existing work on Question Answering from documents that focuses on identifying an answer to a question within a document, we introduce the novel task of identifying the correct entity answer to a given question based on a collection of unstructured reviews describing entities. Our task requires processing $500$ times more documents per question than traditional QA tasks and each document is also larger than those used in existing research. The task is reflective of real world challenges and we use automated methods to generate data for this task. Our experiments suggest that identifying better samples to train,  %reducing the search space, 
and building models specialized for different types of questions may be critical for success on this task. In addition, the use of deeper reasoning methods may be effective but we need to ensure they scale on the size of the dataset. Our best system has an $Acc@3$ of $19.3$\% and is an ensemble consisting of Duet v2 along with a Siamese network that employs curriculum learning with harder negative samples and smaller, but representative documents. This highlights the challenges in the task and scope for advancing QA research. We will make resources from this paper available for further research.

% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||l|l|l|l}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\  \end{tabular}}&{17.63}               &  {23.59}               &            {55.4}     &     {0.166 }     \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (23 epochs) %\end{tabular}}&{\bf }               &  {\bf }               & %           {\bf }     &     {\bf }     \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ CL  \end{tabular}}&{\bf19.28 }               &  {\bf 25.4}               &            {\bf 57.3}     &     {\bf0.173 }     \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance with and without curriculum learning (CL) } \label{tab:curr-learning}
% \end{table}



%Some question answering systems utilize methods such as those used in our baseline models to prune a large search space and then run models with deeper reasoning on a small subset to get 

==> experiments_mausam.tex <==

\section{Experiments}\label{sec:experiments}

We ask the following questions in our experiments: 
(1) What is the performance of the \csr\ model compared to other baselines for this task?
%(2) What is the incremental value of each component used in \csr?
(2) How does the \csr\ model compare with neural IR and neural QA models?
(3) What are the characteristics of questions correctly answered by our system?


%(1) Is constructing the representative document using clustering better than a random sentence selection baseline? 
%(2) To what extent are non-neural baselines such as TF-IDF retrieval, effective for this task? Could they be useful in pruning the search space for a downstream module with deeper reasoning and re-ranking? 
%(3) How do the characteristics of correctly questions correctly answered by a shallow reasoner like Duet differ from a deep reasoner such as QESE? %(2) How well does QESE perform on the full-ranking task?  %(2) In our Question-Entity Siamese (QESE) network, are generating question-dependent entity embeddings helpful? 
%(3) Is constructing the representative document using clustering better than other sentence selection baselines?  %(4) How can the quality of negative samples used in our training be improved? 
%(4) How do state-of-the art neural IR models designed for adhoc-retrieval tasks perform on our task? % for our task?

\vspace{0.5ex}
\noindent{\bf Metrics: }
We use Accuracy@N metrics for evaluating a QA system. 
For a question $q$, let the set of top ranked $N$ entities returned by the system be $E_N$, and let the correct (gold) answer entities for the question be denoted by set $G$. We give credit to a system for Accuracy@N if the sets $E_N$ and $G$ have a non-zero intersection. We also use the standard mean reciprocal rank (MRR) metric. To compute MRR score we only consider the highest ranked gold answer, if multiple gold answers exist for a question.

\begin{comment}
then   $Acc@N = \mathbbm{1} ((E_N \cap G)\neq \phi)$, 
%\begin{equation}
 %   ACC@N = \mathbbm{1} (G \in E_N)  
%\end{equation}
where $\mathbbm{1}$\{\} is the indicator function. We report $Acc@3$, $Acc@5$ and $Acc@30$ scores. 

%Note that our metric 
%the highest rank the gold answer ranks is used compute eas ranking correct answer.
\end{comment}

%\noindent {\bf Mean Reciprocal Rank (MRR): } % For each question we use the highest ranked gold entity to compute MRR.  %Let the set of questions be $Q$, and let $E$ be the ranked list of entities $E$ for a guestion $q$ and $R'_q$ be the list of ranks of the gold entities for the question $q$. Then we define the MRR metric as 
% For a given ranked list of entities $E$, %it is the average of the inverse ranks of each correct answer entity.
% if the entity at rank $r$ is the gold answer entity then the mean reciprocal rank is given by $ $$MRR = \frac{1}{|Q|}\sum_i^{|E|} \frac{1}{r_i}$$.


\begin{comment}
Let $Q$ be the set of questions in our test set and let $r_i$ be the rank of the highest ranked gold entity for question $q_i \in Q$. The mean reciprocal rank (MRR) is then defined as: $\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$.
%\begin{equation}
%$\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$
%\end{equation}
Note that in case of questions with multiple gold entity answers, both metrics use the gold entity with the highest rank.
\end{comment}

\vspace{0.5ex}
\noindent{\bf Hyper-parameter Settings: }
The convolution layers in the Duel model used kernel sizes of $1$ and $3$ for local and distributed interactions respectively. Hidden nodes were initialized with size of input word embeddings, $128$ dimensions. % Questions were truncated at $200$ tokens and entity review documents at $1600$. %The local a kernel size of $3$ for the convolution layers with $128$-dimensional hidden nodes. 
All Reasoning models were trained for 5 days on $6$ K80 GPUs (approx. 14 epochs models) using $10$ negative samples for each QA pair. We used $3$-layer $128$-dimensional bidirectional GRUs to encode questions and review sentences. Input word embeddings were updated during training and USE embeddings returned $512$ dimension embeddings. For all experiments we set $\delta=1$ in our max-margin criterion. We used Adam Optimizer \cite{Adam} with a learning rate of $0.001$ for training. Training the Reasoning model took $11.5$ hours per epoch on 4 K-80 GPUs. % and loss stabilization as stopping criteria.

\subsection{Simple Baselines for our Task}
As discussed previously, existing neural QA models do not scale for task. We therefore,
%Due to scalability requirements of our task, we cannot compare against state of the art QA models. 
compare the performance of \csr\  with several natural baselines for our task. %following telescoping methods:
%We consider the following non-neural models:
%To demonstrate the challenging nature of the task, we present results from baseline systems using BM25 retrieval baselines as well as a few neural retrieval models.
  %To make the task simpler, all methods below only consider candidates that are of the same type as the gold answer and not all possible candidate entities. 
%\subsection{Non-Neural Baselines}

\noindent{\bf Random Entity Baseline:} Returns a random ranking of the candidate answer space.% (of the same type as the gold entity).

\noindent{\bf Ratings Baseline:} Returns a global (question-independent) ranking of candidate entities based on user ratings.

\noindent{\bf BM25 Retrieval:} We index each entity along with its reviews into Lucene\footnote{\emph{http://lucene.apache.org/}}. Each question is transformed into a query using the default query parser that removes stop words and creates a disjunctive term query. Entities are scored and ranked using BM25 ranking \cite{BM25}. Note that this baseline is considered a strong baseline for information retrieval (IR) and is, in general, better than most neural IR models \cite{BM25Good}.  % \cite{BM25} and returned as answers to the question.
% \subsection{Neural Models}
% Since we formulate the task as a ranking problem, we train the model to score a correct answer higher than an incorrect answer \cite{Siamese1,Siamese2}. Specifically, given an entity document ($d_e$) and a question $q$, we generate a score $s_e$ for the entity with respect to $q$ by computing a weighted dot product $s_e$=$qWd_{e}$ and would like $s_p$ $>$ $s_n$ for a correct entity $p$ and an incorrect entity $n$. % All the networks are trained by sampling $10$ negative (incorrect answer) entities for each question-answer pair and using hinge loss 
% This is easily specified to the model by using hinge loss ($max(0,s_p - s_n + \delta$)) between a correct answer ($s_p$) and negative sample ($s_n$) as the objective function. We set $\delta=1$ in our experiments.  %[ ADD HYPER PARAM DETAILS]

\noindent{\bf Review-AVG Model: }
%We experiment with a simple neural baseline. % that uses averaged vector embeddings for sentences to represent each document.
This is a trained model in which questions are encoded using a self-attended bi-directional GRU \cite{intra-attention} to generate a question representation.% $\phi$. %The  encoded sentence representations are then used as input to another bi-directional LSTM with self attention to create the final question representation $q$.
%Due to the extremely large nature of entity documents, learning document representations using sequence models becomes prohibitively expensive.
We then use universal sentence embeddings (USE) \cite{USE2018} to pre-compute vector representations for each sentence and average them to create a document representation. An entity is scored via a weighted dot product between question and document embeddings.
%Let $s_{ij}$ be the $j$th sentence vector in $i$th review. Let $w^{k}_{ij}$ be the $k$th word in sentence $s_{ij}$. 
% For an entity $e$, we create its embedding ($d_e$) by first averaging the embeddings of sentences in a review to create a review embedding and then define the entity representation as an average of the review embeddings. Formally, entity embedding $d_e$ is given by:%$\sum_{i}\frac{\sum_js_{ij}/|S_i|}{|N_e|}$
%\noindent{\bf Duet v2:} The Duet v2 model \cite{DUET2} using the representative documents created using clustering.
% \begin{equation}
% \small
%     \vspace{-1ex}
%     %d_e=\sum_{i}\frac{\sum_j (\gamma_{ij}
%     d_e=\sum_{i}\frac{\sum_j
%     s_{ij}/|S_i|}{|N_e|}
%     \vspace{-1ex}
% \end{equation}

% where $|S_i|$ is the number of sentences in review $i$ and $|N_e|$ is the number of reviews in entity $e$. As before, the model is trained using max-margin criterion, but using $d_e$ as the entity embedding.
%[ NOTATION TO BE STANDARDIZED]
%\noindent{Duet V2 Model:} We use the neural IR model, DUET, \cite{DUET} which was recently improved to incorporate inverse document frequencies as well as word vectors \cite{DUET2}.
%\noindent{\bf Duet V2 Model:} We use the neural IR model, Duet v2 \cite{DUET2}, which is an improved version of Duet \cite{DUET}. % incorporate inverse document frequencies as well as word embeddings \cite{DUET2}.



\begin{table}[]
\centering
%\small
\begin{tabular}{|c||c|c|c|c|}
\hline
\textbf{Method}                                              & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30 } & \textbf{MRR} \\ \hline \hline
\textbf{Random} & 0.35               & 0.48               &    3.98                             &   0.008            \\ %\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Ratings\\ \end{tabular}}  &         0.39        & 0.83                &   3.46                           & 0.007          \\  %\hline  
\textbf{BM25 }   & 6.78                                           &  9.97               &  30.58              &  0.073                                              \\ %\hline 
\textbf{Review-AVG}                                                                 &  {7.97 }              &  {11.91 }              &            {30.9 }     &     {0.084}         \\ %\hline %\hline
\textbf{$\csr$}   & {\bf 40.64}            & {\bf 53.04}               &  {\bf 91.59}               & {\bf 0.369}       \\ \hline     

%\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline

%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Performance of baseline systems and the $\csr$  model on our task. Accuracy report in \%.} \label{tab:expts}
%\vspace*{-3ex}
\end{table}

\subsection{Results}
Table \ref{tab:expts} compares \csr\ against these baselines. We find that
\csr\ massively outperforms all these simple baselines for the task. 
Even the strong baseline of BM25 retrieval, which is commonly in retrieval tasks, is not as effective for this dataset. The neural baseline model, Review-AVG, also performs quite poorly on this task, while our \csr\ model has an Acc@3 of about 41\%. These results underscore the value of \csr\ model for this task.

%We now present an ablation study demonstrating the incremental contributions made by each of our components:% the
%contribution of each of our modeling choices

\subsection{Ablation Study}
\begin{figure*}[ht]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.65]{figs/TourQue_CANDIDATE_SPACE-CSR.jpg}
   %\vspace*{-2ex}
   \caption{Entity class-wise break-up of the number of times (and \%) a correct answer was within the top-3 ranks binned based on the size of candidate search space (X-axis).}
   %\vspace*{-3ex}
   \label{fig:space-study}
 %\end{adjustwidth}
 
 }
%\vspace*{-1ex}
 \end{figure*} 

%We study the effect of incorporating each component used by $\csr$ (i) clustering for generating representative documents (ii) selecting top ranked candidates using a neural IR model (iii) re-ranking using a deep reasoning model.

We now perform an ablation study in which we remove (or replace) one of the components of \csr\ to evaluate the incremental value of each component. This ablation study also helps in assessing the performance of \csr\ against a strong IR model and a strong QA model. 

\subsubsection{Clustering:} We first evaluate the value of the clustering step and creating representative entity documents. Unfortunately, if we give the full entity document instead of a representative one, the neural select-rerank model cannot be trained due to GPU memory limitations. So, in this experiment, we replace the clustering phase with randomly selecting $100$ sentences for an entity. We name this model {\bf $\rsr$}. Table \ref{tab:ablation} shows a 13 pt drop in Accuracy@3 highlighting the importance of finding useful exemplars. We also tried to create document representations by selecting $100$ sentences from an entity document by indexing them in Lucene and then using the question as a query. We found that this method, understandably, returned very few sentences -- the questions (query) are longer than a sentence on average and the lexical gap is too big to overcome with simple expansion techniques. %Working with the complete original documents is also not possible since the documents are too large and do not fit in GPU memory for training.

%We first investigate whether document representations created using sentence clusters performs better than randomly selecting $100$ sentences from an entity. As can be seen from Table \ref{tab:ablation} (Model {\bf $\rsr$}) the use of random sentences result in a significant drop in performance, highlighting the importance of constructing useful exemplars. We also tried to create document representations by selecting $100$ sentences from an entity document by indexing them in Lucene and then using the question as a query. We found that this method, understandably, returned very few sentences -- the questions (query) is longer than a sentence on average and the lexical gap is too big to overcome with simple expansion techniques. Working with the complete original documents is also not possible since the documents are too large and do not fit in GPU memory for training.

\subsubsection{Selection:} We now remove the IR model from \csr. That is, we directly train our Siamese network on the whole candidate set to generate a complete ranking over the answer space. We name this {\bf $\crq$}. As Table \ref{tab:ablation} shows, the performance suffers a steep drop of over 23 points. We attribute this to the fact that training the reasoner is compute intensive, and it is unable to see many negative samples for a question even after a long time of training. Due to this it likely overfits on the seen negatives, but is unable to perform well when the full candidate set is provided. On the other hand, in the complete \csr\ model, the select module shortlists good candidates a priori and the reasoner's job is limited to finding the best ones from the good candidates, which it is able to do better. 

%Instead of using a neural IR model to reduce the candidate space, we could also run a deep-reasoner to directly generate the full-ranking over the answer space. As the results Table \ref{tab:ablation} (Model {\bf $\cs$}) indicate, selecting and reducing the candidate space is a crucial feature of the system. Running the reasoner directly on the complete candidate space results in a steep drop in performance. %We hypoThe reasoning component is does not adequately train on the large 

\subsubsection{Reranking:} Lastly, we remove the reranker, and  simply return the ranking outputted by Duet. We name this {\bf $\cs$}. Table \ref{tab:ablation} again shows significantly reduced accuracy scores, suggesting that the scalable matching of Duet is useful enough for filtering candidate, but not powerful enough to return the best answer. Overall, we find that each component of \csr\ is critical in its ultimately good performance on the task. Moreover, strong IR only and QA only baselines are not as effective as their combination in \csr. 

%one could also return the ranked candidates returned by the neural IR system as the final answer - do we need a reasoner? Table \ref{tab:ablation} (Model {\bf $ \crq $}) shows the performance of the model and it suggests that the shallow semantic matching is useful for filtering candidates but is not powerful enough to return the best answer. Using all three components results in best performance. % that g the Instead of using a neural IR model to reduce the candidate space, we could also run a deep-reasoner to generate the full-ranking over the answer space. As the results Table \ref{tab:ablation} (Model SR) indicate, the selecting and reducing the candidate space is a crucial component.



\begin{table}
\begin{center}
\begin{tabular}{|c||c|c|c|c|}
\hline
\textbf{Method}                                              & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline \hline
\textbf{\csr}    & {\bf 40.64}            & {\bf 53.04}               &  {\bf 91.59}               & {\bf 0.369}       \\ %\hline \hline
\textbf{\csr}    & {\bf }            & {\bf }               &  {\bf }               & {\bf }       \\ %\hline \hline
%\textbf{\rsr}   & 27.52           & 36.19         & 85.82              & 0.269      \\ %\hline %\hline
\textbf{\rsr}   & 11.88            &   17.30       & 52.14               &  0.122     \\ %\hline %\hline%&  
\textbf{\crq}  &  {17.03}               &  {23.65}               &            {54.90}     &     {0.168  } \\
\textbf{\cs} & {18.27}               &  {23.90}               &            {53.70}     &     {0.169 }            \\  %\hline %\hline %&  
\hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA layer\end{tabular}} &  16.60              & 22.6                & 51.7                                  & 0.154             \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ Random Sent. \end{tabular}} & 9.64              &      13.79       &                       37.18           &  0.098            \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ BM25 Sent. \end{tabular}} &                 &                &                                  &              \\ \hline


%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\end{center}
\caption{Ablation Study: Each of our components are critical in solving this task}\label{tab:ablation}
%\vspace*{-2ex}
\end{table}

% \subsection{Representative Documents}
% %We study if our modeling choice of generating question dependent entity embeddings using the QEA layer was useful. In addition,
% We investigate whether document representations created using sentence clusters perform better than randomly selecting $100$ sentences from an entity. As can be seen from Table \ref{tab:ablation} the use of representative sentences result in marked improvement in performance on the full-ranking task. We also tried to create document representations by selecting $100$ sentences from an entity document by indexing them in Lucene and then using the question as a query. We found that this method, understandably, returned very few sentences -- the questions (query) is longer than a sentence on average and the lexical gap is too big to overcome with simple expansion techniques. 


% \subsection{Telescoping} \label{sec:baselines}

% \subsection{Results}
% \begin{table}[]
% \small
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30 } & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Random\\ Entity\end{tabular}} & 0.35               & 0.48               &    3.98                             &   0.008            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Ratings\\ \end{tabular}}  &         0.39        & 0.83                &   3.46                           & 0.007          \\ \hline  
% \textbf{BM25 }   & 6.78                                           &  9.97               &  30.58              &  0.073                                              \\ \hline %\hline
% \textbf{Review-AVG}                                                                 &  {7.97 }              &  {11.91 }              &            {30.9 }     &     {0.084}         \\ \hline
% \textbf{Duet v2}   &  {\bf 18.27}               &  {\bf 23.9}               &            {\bf 53.7 }     &     {\bf 0.169 }            \\ \hline

% %\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance of different telescoping methods (Full-ranking task).} \label{tab:expts}
% \vspace*{-3ex}
% \end{table}

% As can be seen in Table \ref{tab:expts} we find that baselines such as BM25 retrieval that have commonly been used for telescoping are not as effective for this dataset. A neural baseline model, Review-AVG, that uses average sentence embeddings also performs poorly on this task, while the DUET v2 model that uses our representative documents has an Acc@30 of about 54\%. We thus, apply the DUET v2 as our method for telescoping by providing the top-50 candidates returned by DUET v2 for deeper reasoning and re-ranking by QESE. %All subsequent experiments described in the paper use $100$ sentences from our representative documents. %electing from highly rated (reviewed) entities as answers is also ineffective.


% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.8]{figs/TourQue_Loss_Plot.jpg}
%   %\vspace*{-2ex}
%   \caption{Figure showing the trends in average loss for the first 15 epochs of training. }
%   \label{fig:loss}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-1ex}
%  \end{figure}  
 
%\subsection{Improving Training with Curriculum Learning}

%\noindent{\bf Curriculum Learning:} Max-margin ranking models can be sensitive to the quality of negative samples presented to the model while training. %  Consider, Figure \ref{fig:loss} which shows the variation in loss with number of epochs for the models shown in Table \ref{tab:ablation}.
%As we can see, the average loss per epoch follows a similar trend in all three configurations but they have markedly different accuracy. We hypothesize that this is because our models are presented with negative samples that are easy to distinguish from the gold answer. Thus, the model reports low loss early on without needing to learn effectively.
%\subsubsection{Harder Negative Samples}
%Instead of presenting negative samples chosen at random from the candidate space, can we exploit knowledge about entities to give harder samples to the model and help improve its learning? %In a task such as ours, where there are challenges of scale, training faster and better could be useful. 
%One method of selecting harder samples would be to use the gold entity and find entities {\em similar} to it in some latent space and then present the closest entities as negative samples.  In neural settings, candidate embedding space serves as a natural choice for the latent space; negative samples could be generated by sampling from a probability distribution fitted over the distances from the answer embedding.

%We also experiment with two baseline methods of creating entity embeddings: (i) Using the averaged sentence embeddings of the representative documents (AVG. Emb in \ref{tab:curr-style}) (ii) Doc2Vec \cite{doc2vec}. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. %However, we find that both these embeddings spaces result in a skewed distribution with unhelpful samples, and models using these report poorer performance than sampling at random (Table \ref{tab:curr-style}). %and possibly poorer quality embeddings. 
%This highlights the importance of high quality negative samples for our model.

%One could also use task specific embeddings from QESE to model the candidate space, % however, we do not have an obvious method of identifying such negative entities (and embeddings). 
%Using our QESE model directly is also not an option as 
%however, running running our trained model on the the test data takes $2.5$\footnote{Using $4$ K-$80$ GPUs} days. Generating question specific candidate embeddings for each instance while training (which is nearly $10$ times larger) is thus infeasible.   %while using methods such as doc2vec were resulting in a highly peaked distribution 
%We therefore, decide to generate task specific embeddings using our Question-Entity Siamese model but without the QEA layer that learns question independent entity embeddings. Once a model is trained, embeddings can be generated offline and used to generate a probability distribution (per answer entity) for negative sampling.  

%Another source of negative samples can be to use the top-k candidates returned by the telescoping method and serve them as negative samples. DUET v2 is a less complex model is faster to run. We're thus able to execute forward-pass on the complete training dataset to get the top-k samples in a reasonable amount of time. [ QUANTIFY?]%Thus for a given QA pair, we sample the  entities (in the embedding space based on this model) and fit a probability distribution using its distance from the answer entity. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. 
%As can be seen in the last row of Table \ref{tab:curr-style}, training QESE with harder negative samples with curriculum learning helps train a better model, faster. Interestingly, the negative samples from Duet v2 cause the model performance to drop significantly in the epoch-limited training-time available. %As figure \ref{fig:tough-sampling} shows, using curriculum learning helps converge to better accuracy faster\footnote{The best accuracy for the regular model occurs after $23$ epochs (not shown in Figure \ref{fig:tough-sampling}).} than regular training.  

% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157}            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Doc2Vec Emb. \end{tabular}} &    16.77        & 22.73               &                      53.8          & 0.152             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ AVG Emb. \end{tabular}} &  16.46            &  22.33             & 52.2                                 &  0.159            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb. \end{tabular}} &{\bf 17.03}            &  {\bf 23.65}         &            {\bf 54.9}   &     {\bf 0.168}    \\   \\ \hline


% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Curriculum learning (CL) with different entity embedding schemes (Full-ranking task)} \label{tab:curr-style}
% \vspace{-2ex}
% \end{table}
% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA. layer\end{tabular}} &   68.2           &  77.4            &                          94.8        &  0.58            \\ \hline
% \textbf{QESE}   & {69.2}               &  {78.7}               &            {95.2}     &     {0.6 }             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb \end{tabular}} &       {\bf 71.1}      &    {\bf 79.4}           &                     {\bf  95.4}           &      {\bf 0.61 }       \\ \hline


% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Model performance in a reduced candidate space of $100$ entities} \label{tab:small}
% \vspace{-6ex}
% \end{table}
%\subsection{Ensemble Models}
% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{QESE CL}   &  {17.03}               &  {23.65}               &            {54.9}     &     {0.168  }            \\ \hline
% \textbf{Duet v2}   &  {18.27}               &  {23.9}               &            {53.7 }     &     {0.169 }            \\ \hline
% \hline
% \textbf{\begin{tabular}[|c|]{@{}c@{}}QESE CL\\ + Duet v2 \end{tabular}} &{\bf 19.27}            &  {\bf 25.32 }         &            {\bf 54.9 }   &     {\bf 0.177}   \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance of (i) Duet v2 (ii) Ensemble model with QESE CL + Duet v2} \label{tab:duet}
% \end{table}
%\noindent{\bf Full Model:} We evaluate our full model; it uses Duet for pruning the candidate answer space and QESE model trained to re-rank these shortlisted answers. As can be seen in Table \ref{tab:telescope}, the QESE model trained for re-ranking telescoped candidates does significantly better than a QESE model trained for a full-ranking task. We also study whether using an ensemble instead of a pipeline could be better and our results from Tables \ref{tab:expts} and \ref{tab:telescope} suggest that neither Duet nor QESE, on their own, do as well on the full ranking task. In the next section we study the characteristics of the answering space for both models. %we hypothesize that this is because while the models have different strengths on the full ranking 


% \begin{table}[]
% \small
% \begin{tabular}{c||c|c|c|c}
% %\hline
%                                                                       & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline \hline
% %\textbf{\begin{tabular}[c]{@{}l@{}}QESE CL\\ (Task emb.)\end{tabular}} &   23.45             & 34.2               & 81.49                &  0.230            \\ \hline
% {\bf QESE}   &  {17.03}               &  {23.65}               &            {54.9}     &     {0.168  }            \\ \hline
% \textbf{\begin{tabular}[|c|]{@{}c@{}}QESE \\ (+) Duet  Ensemble  \end{tabular}} &{19.27}            &  {25.32 }         &            {54.9 }   &     {0.177}   \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE \\ (Telescope - Duet)\end{tabular}}     &    {\bf 40.64}            & {\bf 53.04}               &  {\bf 91.59}               & {\bf 0.369}       \\ \hline     
% \end{tabular}
% \caption{Performance improvement by using a telescope strategy for re-ranking pruned candidates.}
% \label{tab:telescope}
% \end{table}
%\subsection{Duet v.s. QESE (Full Ranking task)}
%\noindent{\bf Duet v.s. QESE (Full Ranking task):} 
%A deeper study using the validation set reveals that both models have different strengths on the full ranking task. At top-3, they correctly answer different sets of questions; between 45-52\% of the questions answered by one model were not answered by the other\footnote{At top-$30$, the percentage of non-overlapping correctly answered questions reduces to 22-25\%.}. Further, we find that Duet v2 which is a shallow reasoner based on matching local and distributed text representations, gains by correctly answering more 42\% more questions (at top-3) with large candidate spaces. This is the primary reason why telescoping is effective. We also considered building an ensemble of DUET and QESE, both trained on the full ranking task. As Table \ref{tab:telescope} shows it results in only marginal gains over the models. %On other hand, QESE CL, which is a deep reasoner (and thus, slower to train), does not train enough in the same time frame to be as effective in very large search spaces. %Note, however that both models have similar performance when we compare their Acc@5 and Acc@30. %The set of questions answered correctly by both models@30 %Further, about 43\% of the questions answered only by QESE were for hotels and attractions, while for the Duet V2 model it is 27\% -- Duet v2 correctly answers a larger fraction of restaurant questions. 




%We thus, build a simple neural classifier (trained on validation set) that uses the strengths of both models and chooses between the two models for answering. It uses question embeddings from QESE CL along with features to indicate target entity-type and we find that this ensemble model results in improved performance (Table \ref{tab:duet}). 
%To summarize, we find that both, shallow and deep reasoners have different strengths; both models answer  
%[ADD COMMENT ABOUT HOW MULTIPLE MODELS STRENGTHS]

\subsection{Answering Characteristics}
We study the performance of different configurations used in the ablation study. 
%[TO BE UPDATED] 
%[ TO BE UPDATED]
%[ SHOULD THIS INCLUDE OR BE ON FINAL TELESCOPE MODEL?]
%As mentioned earlier, existing QA tasks operate in a much smaller candidate search spaces. In this section we study the role the size of candidate search space might play on model performance. 
The plots in Figure \ref{fig:space-study} show the number of times the gold answer was in the top-3 ranks for questions from each entity class\footnote{Recall that each question has its own candidate space}. The results have been binned based on the size of the candidate space (0-100, 100-1000, 1000+). Questions on restaurants dominate the dataset and also have a larger candidate space with $1,553$ questions in the validation set having a search space greater than $1,000$ candidates. In this sub-class of questions, we find that the $\cs$ model, which does not do deep reasoning, answers more questions correctly in the top-3 ranks, as compared to the $\crq$ model. This observation strengthens our motivation for using a scalable retrieval model to prune the large search space. Using the full model $\csr$ on this class of questions results in a significant boost in performance. 

We find that in hotels and attractions since the search space in most questions isn't as large , both the \cs\ and \crq\ models have comparable performance. However, using the full \csr\ model still shows considerable improvement but the gains are not as big as seen in questions on restaurants. Overall, we find that the reduction of search space is critical for this task and the use of a scalable shallow neural model to reduce the search space is an effective strategy to improve performance.

%Of this, only $385-431$ ($25-28$\%) of the questions are answered correctly in the top-3 ranks. In contrast, questions on hotels and attractions largely have a search space of $1000$ candidates or less. Of these, $50$\% of the questions on hotels are answered correctly in the top-3 ranks while the $59$\% of the questions on attractions are answered correctly. 

%To further highlight how the number of candidate answers affect model performance, we also compared the performance of our models with a smaller candidate space of $100$ entities ($1$ correct and $99$ randomly sampled incorrect entities). A comparison between Table \ref{tab:curr-style} \& Table \ref{tab:small} demonstrates that, not only does a large candidate space cause the performance of all models to suffer, it is also likely that only a small percentage of candidate entities are confusing. Thus, we believe that if we had a scalable and effective method of identifying confusing candidate answers for each question, it could help in training, as well as, in enabling a telescope setting for pruning the search space, as used in existing QA tasks \cite{drqa,R3}. % could be helpful in our task. %This also reinforces our belief that while a majority of the candidates are easy to d

%\subsection{Qualitative Study}
% In order to visualize what our model is learning, we study the attention weights applied to tokens in a question and the review sentences. Figure \ref{fig:attention} shows an example from the validation set. Here, the user is looking for recommendations for places to stay and the review sentences shown are for the top ranked (and correct) entity answer (Marina Bay Sands, Singapore) returned by our system. It is interesting to note that the model focuses on descriptive words in reviews while attempting to rank entities. 

% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.3]{figs/Attention_Visualization_1.jpg}
%   % \vspace*{-2ex}
%   \caption{Visualization of attention weights. Darker colours indicate higher attention weights. Review sentences shown  ranked in order of sentence level attentions. Truncated for ease of presentation.}
%   \label{fig:attention}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-2ex}
%  \end{figure}  

\section{Conclusion}
%In contrast to existing work on Question Answering from documents that focuses on identifying an answer to a question within a document,
In the spirit of defining a question answering challenge that is closer to a real-world QA setting,  we introduce the novel task of identifying the correct entity answer to a given user question based on a collection of unstructured reviews describing entities. We harvest a dataset of over 48,000 QA pairs, which enables end to end training of models.  %The task is reflective of real world challenges and we use automated methods to generate data for this task. 

The biggest challenge in this dataset is that of scalability. Our task requires processing $500$ times more documents per question than most existing QA tasks, and individual documents are also much larger in size.
In response, we develop a cluster-select-rerank architecture that brings together neural IR and QA models for an overall good performance. The neural models work on smaller but representative documents, which appears to be critical for scaling them to this size. Our best system finds a correct answer in top-3 for 40\% of the questions, which is enormously higher than various baseline models, including its own ablated models. 

We believe that further research on this task will significantly improve the state of the art in question answering. A natural extension to our model will be to make clustering step question-dependent. An observation is Accuracy@30 is over 90\%, but only 40\% at 3, suggesting that a better reranker could really improve the performance. A possibility is to use iterative retrieval of sentences from the whole entity document at rerank phase, so that important information is not missed at answering time. We will make resources from this paper available for further research.

%Our experiments suggest %that identifying better samples to train,  %reducing the search space, 
%and 
%building models specialized for different types of questions may be critical for success on this task. In addition, the use of deeper reasoning methods may be effective but we need to ensure they scale on the size of the dataset. Our best system has an $Acc@3$ of $40.64$\% and uses a scalable neural ranker to prune the candidate space before employing a network with deeper reasoning. The neural models we present work on smaller but representative documents which appear to be critical for this task. % curriculum learning with harder negative samples and smaller, but representative documents. 
%Our work highlights the challenges in the task and scope for advancing QA research. We will make resources from this paper available for further research. [ WHAT DO WE SUGGEST FOR FUTURE WORK?]

% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||l|l|l|l}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\  \end{tabular}}&{17.63}               &  {23.59}               &            {55.4}     &     {0.166 }     \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (23 epochs) %\end{tabular}}&{\bf }               &  {\bf }               & %           {\bf }     &     {\bf }     \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ CL  \end{tabular}}&{\bf19.28 }               &  {\bf 25.4}               &            {\bf 57.3}     &     {\bf0.173 }     \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance with and without curriculum learning (CL) } \label{tab:curr-learning}
% \end{table}



%Some question answering systems utilize methods such as those used in our baseline models to prune a large search space and then run models with deeper reasoning on a small subset to get 

==> experiments_shorten.tex <==

\section{Experiments}\label{sec:experiments}

We ask the following questions in our experiments: 
(1) Is constructing the representative document using clustering better than a random sentence selection baseline? 
(2) To what extent are non-neural baselines such as TF-IDF retrieval, effective for this task? Could they be useful in pruning the search space for a downstream module with deeper reasoning and re-ranking? 
(3) How do the characteristics of correctly questions correctly answered by a shallow reasoner like Duet differ from a deep reasoner such as QESE? %(2) How well does QESE perform on the full-ranking task?  %(2) In our Question-Entity Siamese (QESE) network, are generating question-dependent entity embeddings helpful? 
%(3) Is constructing the representative document using clustering better than other sentence selection baselines?  %(4) How can the quality of negative samples used in our training be improved? 
%(4) How do state-of-the art neural IR models designed for adhoc-retrieval tasks perform on our task? % for our task?

\subsection{Metrics}

For a question $q$, let the set of top ranked $N$ entities returned by the system be $E_N$, and let the correct (gold) answer entities for the question be denoted by set $G$, then   $Acc@N = \mathbbm{1} ((E_N \cap G)\neq \phi)$, 
%\begin{equation}
 %   ACC@N = \mathbbm{1} (G \in E_N)  
%\end{equation}
where $\mathbbm{1}$\{\} is the indicator function. We report $Acc@3$, $Acc@5$ and $Acc@30$ scores. 

%Note that our metric 
%the highest rank the gold answer ranks is used compute eas ranking correct answer.

\noindent {\bf Mean Reciprocal Rank (MRR): } % For each question we use the highest ranked gold entity to compute MRR.  %Let the set of questions be $Q$, and let $E$ be the ranked list of entities $E$ for a guestion $q$ and $R'_q$ be the list of ranks of the gold entities for the question $q$. Then we define the MRR metric as 
% For a given ranked list of entities $E$, %it is the average of the inverse ranks of each correct answer entity.
% if the entity at rank $r$ is the gold answer entity then the mean reciprocal rank is given by $ $$MRR = \frac{1}{|Q|}\sum_i^{|E|} \frac{1}{r_i}$$.
Let $Q$ be the set of questions in our test set and let $r_i$ be the rank of the highest ranked gold entity for question $q_i \in Q$. The mean reciprocal rank (MRR) is then defined as: $\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$.
%\begin{equation}
%$\frac{1}{|Q|}\sum_i^{|Q|} \frac{1}{r_i}$
%\end{equation}
Note that in case of questions with multiple gold entity answers, both metrics use the gold entity with the highest rank.

\subsection{Hyper-parameter Settings}
All models were trained for 5 days (approx. 14 epochs \footnote{Trained on $6$ K80 GPUs.} for QESE based models) using $10$ negative samples for each QA pair. We used $3$-layer $128$-dimensional bidirectional GRUs to encode questions and review sentences. Input word embeddings were updated during training and USE embeddings returned $512$ dimension embeddings. For all experiments we set $\delta=1$ in our max-margin criterion. We used Adam Optimizer \cite{Adam} with a learning rate of $0.001$ for training. Training the QESE model  took $11.5$ hours per epoch on 4 K-80 GPUs.% and loss stabilization as stopping criteria.

\begin{figure*}[ht]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.65]{figs/TourQue_CANDIDATE_SPACE-10.jpg}
   %\vspace*{-2ex}
   \caption{Entity class-wise break-up of the number of times (and \%) a correct answer was within the top 10 ranks binned based on the size of candidate search space (X-axis).}
   %\vspace*{-3ex}
   \label{fig:space-study}
 %\end{adjustwidth}
 
 }
%\vspace*{-1ex}
 \end{figure*} 

 \begin{table}[]
\small
\begin{tabular}{c||l|l|l|l}
\textbf{Method}                                              & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline \hline
\textbf{QESE}   &{\bf 17.03}            &  {\bf 23.65}         &            {\bf 54.9}   &     {\bf 0.168}  \\ \hline %&  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA layer\end{tabular}} &  16.60              & 22.6                & 51.7                                  & 0.154             \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ Random Sent. \end{tabular}} & 9.64              &      13.79       &                       37.18           &  0.098            \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ BM25 Sent. \end{tabular}} &                 &                &                                  &              \\ \hline


%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Effectiveness of representative documents (Full-ranking task)} \label{tab:ablation}
\vspace*{-2ex}
\end{table}

\subsection{Representative Documents}
%We study if our modeling choice of generating question dependent entity embeddings using the QEA layer was useful. In addition,
We investigate whether document representations created using sentence clusters perform better than randomly selecting $100$ sentences from an entity. As can be seen from Table \ref{tab:ablation} the use of representative sentences result in marked improvement in performance on the full-ranking task. We also tried to create document representations by selecting $100$ sentences from an entity document by indexing them in Lucene and then using the question as a query. We found that this method, understandably, returned very few sentences -- the questions (query) is longer than a sentence on average and the lexical gap is too big to overcome with simple expansion techniques. 


\subsection{Telescoping} \label{sec:baselines}
We compare the following telescoping methods:
%We consider the following non-neural models:
%To demonstrate the challenging nature of the task, we present results from baseline systems using BM25 retrieval baselines as well as a few neural retrieval models.
 
 %To make the task simpler, all methods below only consider candidates that are of the same type as the gold answer and not all possible candidate entities. 
%\subsection{Non-Neural Baselines}
\noindent{\bf Random Entity Baseline:} Returns a random ranking of the candidate entity space.% (of the same type as the gold entity).

\noindent{\bf Ratings Baseline:} Returns a ranking of the candidate entities based on user review-ratings.

\noindent{\bf BM25 Retrieval:} We index each entity along with its reviews into Lucene\footnote{http://lucene.apache.org/}. Each question is transformed into a query using the default query parser that removes stop words and creates a disjunctive term query. Entities are scored and ranked using BM25 ranking \cite{BM25}. Note that this baseline is considered a strong baseline for information retrieval (IR) and is, in general, better than most neural IR models \cite{BM25Good}.  % \cite{BM25} and returned as answers to the question.
% \subsection{Neural Models}
% Since we formulate the task as a ranking problem, we train the model to score a correct answer higher than an incorrect answer \cite{Siamese1,Siamese2}. Specifically, given an entity document ($d_e$) and a question $q$, we generate a score $s_e$ for the entity with respect to $q$ by computing a weighted dot product $s_e$=$qWd_{e}$ and would like $s_p$ $>$ $s_n$ for a correct entity $p$ and an incorrect entity $n$. % All the networks are trained by sampling $10$ negative (incorrect answer) entities for each question-answer pair and using hinge loss 
% This is easily specified to the model by using hinge loss ($max(0,s_p - s_n + \delta$)) between a correct answer ($s_p$) and negative sample ($s_n$) as the objective function. We set $\delta=1$ in our experiments.  %[ ADD HYPER PARAM DETAILS]

\noindent{\bf Review-AVG Model}
%We experiment with a simple neural baseline. % that uses averaged vector embeddings for sentences to represent each document.
Questions are encoded using a self-attended bi-directional GRU \cite{intra-attention} to generate a question representation.% $\phi$. %The  encoded sentence representations are then used as input to another bi-directional LSTM with self attention to create the final question representation $q$.
%Due to the extremely large nature of entity documents, learning document representations using sequence models becomes prohibitively expensive.
We then use universal sentence embeddings (USE) \cite{USE2018} to pre-compute vector representations for each sentence and use them to create the document representations. %Let $s_{ij}$ be the $j$th sentence vector in $i$th review. Let $w^{k}_{ij}$ be the $k$th word in sentence $s_{ij}$. 
% For an entity $e$, we create its embedding ($d_e$) by first averaging the embeddings of sentences in a review to create a review embedding and then define the entity representation as an average of the review embeddings. Formally, entity embedding $d_e$ is given by:%$\sum_{i}\frac{\sum_js_{ij}/|S_i|}{|N_e|}$
%\noindent{\bf Duet v2:} The Duet v2 model \cite{DUET2} using the representative documents created using clustering.
% \begin{equation}
% \small
%     \vspace{-1ex}
%     %d_e=\sum_{i}\frac{\sum_j (\gamma_{ij}
%     d_e=\sum_{i}\frac{\sum_j
%     s_{ij}/|S_i|}{|N_e|}
%     \vspace{-1ex}
% \end{equation}

% where $|S_i|$ is the number of sentences in review $i$ and $|N_e|$ is the number of reviews in entity $e$. As before, the model is trained using max-margin criterion, but using $d_e$ as the entity embedding.
%[ NOTATION TO BE STANDARDIZED]
%\noindent{Duet V2 Model:} We use the neural IR model, DUET, \cite{DUET} which was recently improved to incorporate inverse document frequencies as well as word vectors \cite{DUET2}.
%\noindent{\bf Duet V2 Model:} We use the neural IR model, Duet v2 \cite{DUET2}, which is an improved version of Duet \cite{DUET}. % incorporate inverse document frequencies as well as word embeddings \cite{DUET2}.



\subsection{Results}
\begin{table}[]
\small
\begin{tabular}{c||c|c|c|c}
\textbf{Method}                                              & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30 } & \textbf{MRR} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Random\\ Entity\end{tabular}} & 0.35               & 0.48               &    3.98                             &   0.008            \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Ratings\\ \end{tabular}}  &         0.39        & 0.83                &   3.46                           & 0.007          \\ \hline  
\textbf{BM25 }   & 6.78                                           &  9.97               &  30.58              &  0.073                                              \\ \hline %\hline
\textbf{Review-AVG}                                                                 &  {7.97 }              &  {11.91 }              &            {30.9 }     &     {0.084}         \\ \hline
\textbf{Duet v2}   &  {\bf 18.27}               &  {\bf 23.9}               &            {\bf 53.7 }     &     {\bf 0.169 }            \\ \hline

%\textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157  }            \\ \hline

%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
%\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
\end{tabular}
\caption{Performance of different telescoping methods (Full-ranking task).} \label{tab:expts}
\vspace*{-3ex}
\end{table}

As can be seen in Table \ref{tab:expts} we find that baselines such as BM25 retrieval that have commonly been used for telescoping are not as effective for this dataset. A neural baseline model, Review-AVG, that uses average sentence embeddings also performs poorly on this task, while the DUET v2 model that uses our representative documents has an Acc@30 of about 54\%. We thus, apply the DUET v2 as our method for telescoping by providing the top-50 candidates returned by DUET v2 for deeper reasoning and re-ranking by QESE. %All subsequent experiments described in the paper use $100$ sentences from our representative documents. %electing from highly rated (reviewed) entities as answers is also ineffective.


% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.8]{figs/TourQue_Loss_Plot.jpg}
%   %\vspace*{-2ex}
%   \caption{Figure showing the trends in average loss for the first 15 epochs of training. }
%   \label{fig:loss}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-1ex}
%  \end{figure}  
 
%\subsection{Improving Training with Curriculum Learning}

%\noindent{\bf Curriculum Learning:} Max-margin ranking models can be sensitive to the quality of negative samples presented to the model while training. %  Consider, Figure \ref{fig:loss} which shows the variation in loss with number of epochs for the models shown in Table \ref{tab:ablation}.
%As we can see, the average loss per epoch follows a similar trend in all three configurations but they have markedly different accuracy. We hypothesize that this is because our models are presented with negative samples that are easy to distinguish from the gold answer. Thus, the model reports low loss early on without needing to learn effectively.
%\subsubsection{Harder Negative Samples}
%Instead of presenting negative samples chosen at random from the candidate space, can we exploit knowledge about entities to give harder samples to the model and help improve its learning? %In a task such as ours, where there are challenges of scale, training faster and better could be useful. 
%One method of selecting harder samples would be to use the gold entity and find entities {\em similar} to it in some latent space and then present the closest entities as negative samples.  In neural settings, candidate embedding space serves as a natural choice for the latent space; negative samples could be generated by sampling from a probability distribution fitted over the distances from the answer embedding.

%We also experiment with two baseline methods of creating entity embeddings: (i) Using the averaged sentence embeddings of the representative documents (AVG. Emb in \ref{tab:curr-style}) (ii) Doc2Vec \cite{doc2vec}. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. %However, we find that both these embeddings spaces result in a skewed distribution with unhelpful samples, and models using these report poorer performance than sampling at random (Table \ref{tab:curr-style}). %and possibly poorer quality embeddings. 
%This highlights the importance of high quality negative samples for our model.

%One could also use task specific embeddings from QESE to model the candidate space, % however, we do not have an obvious method of identifying such negative entities (and embeddings). 
%Using our QESE model directly is also not an option as 
%however, running running our trained model on the the test data takes $2.5$\footnote{Using $4$ K-$80$ GPUs} days. Generating question specific candidate embeddings for each instance while training (which is nearly $10$ times larger) is thus infeasible.   %while using methods such as doc2vec were resulting in a highly peaked distribution 
%We therefore, decide to generate task specific embeddings using our Question-Entity Siamese model but without the QEA layer that learns question independent entity embeddings. Once a model is trained, embeddings can be generated offline and used to generate a probability distribution (per answer entity) for negative sampling.  

%Another source of negative samples can be to use the top-k candidates returned by the telescoping method and serve them as negative samples. DUET v2 is a less complex model is faster to run. We're thus able to execute forward-pass on the complete training dataset to get the top-k samples in a reasonable amount of time. [ QUANTIFY?]%Thus for a given QA pair, we sample the  entities (in the embedding space based on this model) and fit a probability distribution using its distance from the answer entity. We employ curriculum learning, slowly increasing the selection probability of hard negatives up to a maximum of $0.6$. 
%As can be seen in the last row of Table \ref{tab:curr-style}, training QESE with harder negative samples with curriculum learning helps train a better model, faster. Interestingly, the negative samples from Duet v2 cause the model performance to drop significantly in the epoch-limited training-time available. %As figure \ref{fig:tough-sampling} shows, using curriculum learning helps converge to better accuracy faster\footnote{The best accuracy for the regular model occurs after $23$ epochs (not shown in Figure \ref{fig:tough-sampling}).} than regular training.  

% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{QESE}   &  {16.25}               &  {22.6}               &            {53.8 }     &     {0.157}            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Doc2Vec Emb. \end{tabular}} &    16.77        & 22.73               &                      53.8          & 0.152             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ AVG Emb. \end{tabular}} &  16.46            &  22.33             & 52.2                                 &  0.159            \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb. \end{tabular}} &{\bf 17.03}            &  {\bf 23.65}         &            {\bf 54.9}   &     {\bf 0.168}    \\   \\ \hline


% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Curriculum learning (CL) with different entity embedding schemes (Full-ranking task)} \label{tab:curr-style}
% \vspace{-2ex}
% \end{table}
% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (-) QEA. layer\end{tabular}} &   68.2           &  77.4            &                          94.8        &  0.58            \\ \hline
% \textbf{QESE}   & {69.2}               &  {78.7}               &            {95.2}     &     {0.6 }             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE CL\\ Task Emb \end{tabular}} &       {\bf 71.1}      &    {\bf 79.4}           &                     {\bf  95.4}           &      {\bf 0.61 }       \\ \hline


% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Model performance in a reduced candidate space of $100$ entities} \label{tab:small}
% \vspace{-6ex}
% \end{table}
%\subsection{Ensemble Models}
% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||c|c|c|c}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{QESE CL}   &  {17.03}               &  {23.65}               &            {54.9}     &     {0.168  }            \\ \hline
% \textbf{Duet v2}   &  {18.27}               &  {23.9}               &            {53.7 }     &     {0.169 }            \\ \hline
% \hline
% \textbf{\begin{tabular}[|c|]{@{}c@{}}QESE CL\\ + Duet v2 \end{tabular}} &{\bf 19.27}            &  {\bf 25.32 }         &            {\bf 54.9 }   &     {\bf 0.177}   \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance of (i) Duet v2 (ii) Ensemble model with QESE CL + Duet v2} \label{tab:duet}
% \end{table}
\noindent{\bf Full Model:} We evaluate our full model; it uses Duet for pruning the candidate answer space and QESE model trained to re-rank these shortlisted answers. As can be seen in Table \ref{tab:telescope}, the QESE model trained for re-ranking telescoped candidates does significantly better than a QESE model trained for a full-ranking task. We also study whether using an ensemble instead of a pipeline could be better and our results from Tables \ref{tab:expts} and \ref{tab:telescope} suggest that neither Duet nor QESE, on their own, do as well on the full ranking task. In the next section we study the characteristics of the answering space for both models. %we hypothesize that this is because while the models have different strengths on the full ranking 


\begin{table}[]
\small
\begin{tabular}{c||c|c|c|c}
%\hline
                                                                       & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@30} & \textbf{MRR} \\ \hline \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}QESE CL\\ (Task emb.)\end{tabular}} &   23.45             & 34.2               & 81.49                &  0.230            \\ \hline
{\bf QESE}   &  {17.03}               &  {23.65}               &            {54.9}     &     {0.168  }            \\ \hline
\textbf{\begin{tabular}[|c|]{@{}c@{}}QESE \\ (+) Duet  Ensemble  \end{tabular}} &{19.27}            &  {25.32 }         &            {54.9 }   &     {0.177}   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}QESE \\ (Telescope - Duet)\end{tabular}}     &    {\bf 40.64}            & {\bf 53.04}               &  {\bf 91.59}               & {\bf 0.369}       \\ \hline     
\end{tabular}
\caption{Performance improvement by using a telescope strategy for re-ranking pruned candidates.}
\label{tab:telescope}
\end{table}
\subsection{Duet v.s. QESE (Full Ranking task)}
%\noindent{\bf Duet v.s. QESE (Full Ranking task):} 
A deeper study using the validation set reveals that both models have different strengths on the full ranking task. At top-3, they correctly answer different sets of questions; between 45-52\% of the questions answered by one model were not answered by the other\footnote{At top-$30$, the percentage of non-overlapping correctly answered questions reduces to 22-25\%.}. Further, we find that Duet v2 which is a shallow reasoner based on matching local and distributed text representations, gains by correctly answering more 42\% more questions (at top-3) with large candidate spaces. This is the primary reason why telescoping is effective. We also considered building an ensemble of DUET and QESE, both trained on the full ranking task. As Table \ref{tab:telescope} shows it results in only marginal gains over the models. %On other hand, QESE CL, which is a deep reasoner (and thus, slower to train), does not train enough in the same time frame to be as effective in very large search spaces. %Note, however that both models have similar performance when we compare their Acc@5 and Acc@30. %The set of questions answered correctly by both models@30 %Further, about 43\% of the questions answered only by QESE were for hotels and attractions, while for the Duet V2 model it is 27\% -- Duet v2 correctly answers a larger fraction of restaurant questions. 




%We thus, build a simple neural classifier (trained on validation set) that uses the strengths of both models and chooses between the two models for answering. It uses question embeddings from QESE CL along with features to indicate target entity-type and we find that this ensemble model results in improved performance (Table \ref{tab:duet}). 
%To summarize, we find that both, shallow and deep reasoners have different strengths; both models answer  
%[ADD COMMENT ABOUT HOW MULTIPLE MODELS STRENGTHS]

\noindent{\bf Effect of size of candidate space:}
%[TO BE UPDATED] 
[ SHOULD THIS INCLUDE OR BE ON FINAL TELESCOPE MODEL?]
As mentioned earlier, existing QA tasks operate in a much smaller candidate search spaces. In this section we study the role the size of candidate search space might play on model performance. The plots in Figure \ref{fig:space-study} show the number of times the gold answer was in the top-10 ranks for questions from each entity class\footnote{Recall that each question has its own candidate space}. The results have been binned based on the size of the candidate space ($0-100$,$100-1000$,$1000+$). Questions on restaurants dominate the dataset and also have a larger candidate space with $1553$ questions in the validation set having a search space greater than $1000$ candidates. Of this, only $385-431$ ($25-28$\%) of the questions are answered correctly in the top-10 ranks. In contrast, questions on hotels and attractions largely have a search space of $1000$ candidates or less. Of these, $50$\% of the questions on hotels are answered correctly in the top-10 ranks while the $59$\% of the questions on attractions are answered correctly. 

%To further highlight how the number of candidate answers affect model performance, we also compared the performance of our models with a smaller candidate space of $100$ entities ($1$ correct and $99$ randomly sampled incorrect entities). A comparison between Table \ref{tab:curr-style} \& Table \ref{tab:small} demonstrates that, not only does a large candidate space cause the performance of all models to suffer, it is also likely that only a small percentage of candidate entities are confusing. Thus, we believe that if we had a scalable and effective method of identifying confusing candidate answers for each question, it could help in training, as well as, in enabling a telescope setting for pruning the search space, as used in existing QA tasks \cite{drqa,R3}. % could be helpful in our task. %This also reinforces our belief that while a majority of the candidates are easy to d

%\subsection{Qualitative Study}
% In order to visualize what our model is learning, we study the attention weights applied to tokens in a question and the review sentences. Figure \ref{fig:attention} shows an example from the validation set. Here, the user is looking for recommendations for places to stay and the review sentences shown are for the top ranked (and correct) entity answer (Marina Bay Sands, Singapore) returned by our system. It is interesting to note that the model focuses on descriptive words in reviews while attempting to rank entities. 

% \begin{figure}[ht]
%  {\footnotesize
%  %\begin{adjustwidth}{-2.2cm}{}
%  %  Requires \usepackage{graphicx}
%  \center
%   \includegraphics[scale=0.3]{figs/Attention_Visualization_1.jpg}
%   % \vspace*{-2ex}
%   \caption{Visualization of attention weights. Darker colours indicate higher attention weights. Review sentences shown  ranked in order of sentence level attentions. Truncated for ease of presentation.}
%   \label{fig:attention}
%  %\end{adjustwidth}
 
%  }
%  \vspace*{-2ex}
%  \end{figure}  

\section{Conclusion}
In contrast to existing work on Question Answering from documents that focuses on identifying an answer to a question within a document, we introduce the novel task of identifying the correct entity answer to a given question based on a collection of unstructured reviews describing entities. Our task requires processing $500$ times more documents per question than traditional QA tasks and each document is also larger than those used in existing research. The task is reflective of real world challenges and we use automated methods to generate data for this task. Our experiments suggest %that identifying better samples to train,  %reducing the search space, 
%and 
building models specialized for different types of questions may be critical for success on this task. In addition, the use of deeper reasoning methods may be effective but we need to ensure they scale on the size of the dataset. Our best system has an $Acc@3$ of $40.64$\% and uses Duet v2 to prune the candidate space before employing a Siamese network with deeper reasoning. The neural models we present work on smaller but representative documents which appear to be critical for this task. % curriculum learning with harder negative samples and smaller, but representative documents. 
Our work highlights the challenges in the task and scope for advancing QA research. We will make resources from this paper available for further research.

% \begin{table}[]
% \scriptsize
% \begin{tabular}{c||l|l|l|l}
% \textbf{Method}                                              & \textbf{Acc@3(\%)} & \textbf{Acc@5(\%)} & \textbf{Acc@30 (\%)} & \textbf{MRR} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\  \end{tabular}}&{17.63}               &  {23.59}               &            {55.4}     &     {0.166 }     \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ (23 epochs) %\end{tabular}}&{\bf }               &  {\bf }               & %           {\bf }     &     {\bf }     \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}QESE\\ CL  \end{tabular}}&{\bf19.28 }               &  {\bf 25.4}               &            {\bf 57.3}     &     {\bf0.173 }     \\ \hline

% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ AVG\end{tabular}} &       0.6          & 1.19                 &   6.04                               & 0.06              \\ \hline
% %\textbf{\begin{tabular}[c]{@{}c@{}}TFIDF\\ MAX\end{tabular}}  &      0.8          & 1.52                 & 7.3                                & 0.014      fthe      \\ \hline \hline 
% \end{tabular}
% \caption{Performance with and without curriculum learning (CL) } \label{tab:curr-learning}
% \end{table}



%Some question answering systems utilize methods such as those used in our baseline models to prune a large search space and then run models with deeper reasoning on a small subset to get 

==> intro_shorten.tex <==
\section{Introduction} \label{sec:introduction}
Recent question answering tasks such as those based on reading comprehension require answers to be generated either based on a single passage, or after reasoning over multiple passages (or small-sized documents) (e.g. {\em SQuAD} \cite{SqUAD}, {\em HotpotQA} \cite{HotpotQA}, {\em NewsQA} \cite{NewsQA}). Answers to questions are assumed to be stated explicitly in the documents \cite{SqUAD} and can be derived with single or multi-hop reasoning over sentences mentioning facts \cite{HotpotQA}. Other variants of these tasks add an additional layer of complexity where the document containing the answer may not be known and needs to be retrieved from a large corpus before answers can be extracted/generated (e.g. {\em SearchQA} \cite{SearchQA}, {\em MS MARCO} \cite{MSMARCO}, {\em TriviaQA} \cite{TriviaQA}). %Such tasks that rely unstructured knowledge as answering source assume answers are stated explicitly in the documents \cite{SqUAD,TriviaQA} or require inference over text from one or more passages/articles to generate the exact correct answer%. Other datasets  to be fetched and then have answers generated from them.  
%Recent question answering datasets focus on a variety of tasks such as passage reading comprehension (e.g. SQuAD \cite{SqUAD}, SearchQA \cite{SearchQA}, NewsQA \cite{NewsQA}, TriviaQA \cite{TriviaQA}, HotpotQA \cite{HotpotQA}), Science Question Answering \cite{OpenBookQA2018,ExplanationBank,AI2}, QA using knowledge graphs \cite{WebQuestions,SimpleQuestions,QuizBowl}, Dialog and Sequential QA (e.g. \cite{dinan2018wizard}, QuAC \cite{QuAC}, CoQA \cite{CoQA}, QBLink \cite{QBLink}), Long Form QA \cite{LongFormQA} that requires abstractive or extractive summary answers. Many existing QA tasks that rely on unstructured knowledge are largely formulated as variants of reading comprehension tasks, which assume answers are stated explicitly in the documents \cite{SqUAD,TriviaQA} or require inference over text from one or more passages/articles to generate the exact correct answer \cite{HotpotQA,CoQA,QuAC,LongFormQA}. 
While these datasets have been useful in furthering research in comprehension, inference and reasoning, we find that they do not always reflect 
% the complex nature of real world information seeking QA. 
% Edited to the following by Krunal
all the complexities of real-world question answering.

% Aditi : Can we remove the duplicate use of 'real world' here? 
%
%Real world questions, 
% for instance, 
% Edited to the following by Krunal
%
%such as those seen on online forums are often verbose, requiring us to first determine what is crucial in the question for answering.  Further, answering such questions is also challenging,  as it could also involve reasoning across large unstructured documents.
\begin{figure*}[h]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.4]{figs/MSEQ_example.jpg}
%   \vspace*{-3ex}
   \caption{\small Question from an online travel forum. Figure from \cite{MSEQPaper}}
   \label{fig:queryExample}
 %\end{adjustwidth}
 }
%\vspace*{-2ex}
 \end{figure*}
For example, consider the question in Figure \ref{fig:queryExample}. Here the user describes {\em who they are}, {\em what they are looking for}, as well as 
% describe their {\em preferences}
% Edited to the following by Krunal
{\em their preferences} for the expected answer.
%
They also mention that they are {\em looking forward to the trip} and are going to be {\em first time visitors} to the city.  %\cite{SqUAD,RetrieveAndReadCIKM}.
% Krunal: Citation problem I think, please check
Answering such questions requires understanding the relevant parts of the question, 
reading information about each candidate answer entity in travel articles, blogs or reviews (\emph{entity documents}), matching relevant question parts with entity documents, and ranking each candidate answer based on the degree of match. 

The foremost challenge in building a QA system for this task is model scalability. Typical QA algorithms apply cross-attention between question and candidate answer texts, which will not scale in our case where entities may have long entity documents (see Table \ref{tab:related} for comparison of document sizes across different QA datasets).  Moreover, the candidate answer spaces for this problem are very high (e.g., New York has tens of thousands of restaurants to choose from), affecting scalability further. There are other technical challenges as well -- the entity documents include reviews written by users, which can be informal and noisy, and may contain subjective contradictory opinions. An entity document may even discuss other entities (e.g., for comparison), making reasoning even harder. Finally, not all aspects of the question are relevant for answering which makes identifying the informational need challenging. It is worth noting that the question in Figure \ref{fig:queryExample} is almost as large as the reading comprehension paragraphs used in tasks such as SQuAD.\footnote{Average size of paragraphs in SQuAD is 140 tokens}

\begin{comment}
Answering such questions requires 
% the creation of a real world knowledge 
% Edited to the following by Krunal
understanding knowledge sources which
%
describe possible answer entities in an unstructured or semi-structured form. Knowledge could come from travel articles, blogs, reviews or similar documents.  %A key difference between answering such questions as compared to existing work is that answers are unlikely to be specified explicitly in knowledge. 
%Most existing QA tasks that rely on unstructured knowledge are largely formulated as variants of reading comprehension tasks, which assume answers are stated explicitly in the documents \cite{SqUAD,TriviaQA} or require inference over text from one or more passages/articles to generate the exact correct answer \cite{HotpotQA,CoQA,QuAC}. These assumptions may not hold always in real world. 
Online reviews describing entities of interest can often be informal and noisy, contain subjective opinions, as well as, sentences unrelated to the entity being considered and in some cases, even discuss other entities (e.g., for comparison). %(e.g. when users draw comparisons).
Further, review collections describing entities can be orders of magnitude larger than articles/documents used in %considered large in 
existing QA tasks (see Table \ref{tab:related}) which also brings in challenges associated with scaling unstructured knowledge understanding. Thus, a QA system for this task would need to process thousands of subjective opinion documents (reviews) to
% Aditi : offer a suggestion (entity) 
suggest an entity
as an answer, making the reasoning task harder. %In addition, in contrast to existing tasks where documents contain an answer to a question, this task would involve reading thousands of documents (each describing an entity), to select the best entity answer. Note that this also translates to a weaker signal for supervision as compared to reading comprehension/answer selection tasks, where an explicit answer is marked or identified in a document.  %(See Table \ref{tab:related}). 
% Edited to the following by Krunal
% existing QA models.
%
%(see section \ref{sec:data}).
%\subsection{Contribution}\\
\end{comment}

\begin{table*}[]
\scriptsize
\center
\begin{tabular}{c|c|c|c|c|c}
\textbf{Dataset} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Knowledge\\ Source\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Answer \\ type\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg. tokens\\ in documents\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Answer \\ document\\ known\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Multiple docs* \\ required\\ for answering\end{tabular}}}  \\ \hline \hline
\textbf{SQuAD} \cite{SqUAD}        & Wikipedia paragraphs                                                                                         &  Span                                                                                    &  137                                                                                               & Y  & N                                                                                             \\
\textbf{NewsQA}\cite{NewsQA}        & CNN News articles                                                                                        &   Span                                                                                  &  $\approx$ 300                                                                                               & Y  & N                                                                                               \\
\textbf{SearchQA} \cite{SearchQA}       & Web snippets                                                                                        &  Span                                                                                   &  25-46                                                                                               &    N & N                                                                                           \\
\textbf{RACE} \cite{RACE}       & Passages on topics                                                                                        &  Choices                                                                                & 350                                                                                                 & Y               &  N                                                                                \\
\textbf{OpenBookQA} \cite{OpenBookQA2018}       & Fact sentences                                                                                        &  Choices                                                                                &   10                                                                                             & Y               &  Y                                                                                \\
\textbf{MSMARCO} \cite{MSMARCO}       &   Web article snippets                                                                                     &  Free text                                                                                   & 10                                                                                                & N         & Y                                                                                      \\
\textbf{MedQA} \cite{MedQA}        & Medical Articles                                                                                        & Choices                                                                                    &  35                                                                                               & Y              & Y                                                                                 \\
\textbf{WikiReading} \cite{WikiReading}        &  Wikipedia articles                                                                                      & Infobox property                                                                                    &                                                                                         489       &    N                  &    N                                                                       \\
\textbf{TriviaQA} \cite{TriviaQA}        &  Web articles                                                                                       &  Span                                                                                   & 2895$^{\dagger}$                                                                                       & N & Y \\
%\textbf{WikiMovies}        &                                                                                         &                                                                                     &                                                                                                 &                                                                               &                   \\
\textbf{HotPot-QA} \cite{HotpotQA}        & Wikipedia paragraphs                                                                                         & Span                                                                                    &        $\approx$ 300                                                                                         &  N                                                                & Y                               \\
\textbf{ELI5} \cite{LongFormQA}         &  Passages on topics                                                                                       &    Free text                                                                              &                                                                                 858                &     Y                                                                       &    N                \\

\hline
Dialog QA - \textbf{QuAC} \cite{QuAC}         &  Wikipedia passages                                                                                       &    Span                                                                              &                                                                                               401  &     Y                                                                        &    N                \\ 

Dialog QA - \textbf{CoQA} \cite{CoQA}         &  Passages on topics                                                                                       &    Free text                                                                              &                                                                                 271                &     Y                                                                       &    N                \\ 


\textbf{Our Dataset}       &  Reviews                                                                                       & Entity (doc.)                                                                                    &                                                                                  3266 & N & Y %excluding empty entities               & N                                                                             & Y                   \\
\end{tabular}
\vspace*{-1ex}
\caption{\small Related datasets on Machine reading/QA and their characteristics. For reading comprehension tasks, the document containing the actual answer may not always be known. *"docs" refers to what the task would consider as its document (e.g., fact sentences for OpenBookQA). $^{\dagger}$Most questions in TriviaQA are answerable using only the first few hundred tokens in the document.} %[t TODO:LAST TWO COLUMNS NEED TO BE DOUBLE CHECKED, ADITI TO COMPLETE TABLE]}  
\label{tab:related}
\vspace*{-5ex}
\end{table*}

%\vspace{0.5ex}
\noindent{\bf Contributions: } 
 We introduce the novel task of answering entity-seeking recommendation questions using a collection of reviews describing entities. It is inspired by the recent work on parsing  multi-sentence  questions \cite{MSEQPaper}. Our work differs from theirs, because they do not attempt to solve this QA task end-to-end and, instead, rely on a pipeline of semantic parsing and querying into a Web API. In contrast, we harvest a novel dataset of tourism questions consisting of $48,147$ QA pairs collected from online travel forums. Each QA pair consists of a question and an answer entity ID, which corresponds to one of the over $200,000$ entity review documents collected from the Web. 
 The entities in our dataset are
hotels, restaurants and general attractions of interest in $50$ cities across the world. 
%Answers to questions in our dataset are different from factual assertions and are {\em subjective}. 
Gold-answer entities are extracted from mentions in full text user responses to the actual forum post.  To the best of our knowledge, we are the first to propose and attempt such an end-to-end task using a collection of entity reviews.

We also present our solution that addresses some of the challenges in our task. In addition to a QA task, our task can also be viewed as an instance of  information retrieval (IR), since we wish to return entity documents (equivalent to returning entities), except that the query is a long question. IR models are more scalable, as they often have methods aimed at primarily matching and aggregating information \cite{IRSurvey}. Thus, these models typically do not achieve deep reasoning, which QA models do, but as mentioned previously, deeper reasoning in QA models (eg. using multiple layers of cross attention) makes them less scalable. We propose a Cluster-Select-Rerank (\csr) architecture for our task, drawing from strengths of both.

\csr's \emph{cluster} step clusters sentences of each entity document in embedding space and picks exemplar sentences to create smaller representative documents for each entity. This reduces document sizes by 70\% and helps improve scalability. Its \emph{select} step trains a fast and scalable CNN-based neural IR method, Duet \cite{DUET2}, to provide a preliminary ranking of all candidate entities. The top entities returned by Duet are selected for deeper reasoning by the \emph{rerank} step, which uses cross attention between question and entity documents to provide a final score for each selected entity. Our experiments demonstrate that using \csr's three step architecture results in better performance (over 25\% relative improvement in Accuracy@3) than relying only on either retrieval or deeper reasoning. 

%Similar to existing work on question-answering from large collections, we rely on a retrieve-rerank style (telescopic) architecture in which a scalable model first reduces the candidate space before deeper reasoning models are applied \cite{IRSurvey}. However, methods such as BM25 \cite{BM25} which are frequently used for pruning the search space are not as effective on our data due to both, the size of the questions as well as, the nature of entity documents. 

%Thus, in order to directly apply neural models on our entity document collection, we create smaller representative documents by clustering sentences for each document in embedding space. This reduces the document size by 70\% and helps improve scalability. We then use a fast and scalable neural retrieval method, Duet \cite{DUET2}, which uses shallow semantic matching based on local and distributed representations of  text, to prune the candidate space on the reduced collection.  Lastly, we use a deeper reasoning neural model to re-rank the pruned candidates and return the final answer. We find that commonly used architectures such BiDAF \cite{BIDAF} and BERT \cite{BERT} which have multiple layers of cross-attention are still prohibitively expensive to run despite the reduction in document size. Our experiments demonstrate that using our three step reduce, retrieve, rerank architecture results in better performance than relying only on either retrieval or deeper reasoning (due to challenges associated with training at scale).% The models with deeper reasoning, despite being simpler than models such as BiDAF \cite{BIDAF} are still expensive to run and do not train adequatley 
%Our final model has an Accuracy@3 of $40$\%.

%Thus,  such as one based on multiple layers of cross attention for reasoning re-ranks the reduced candidate space to return the final answer \cite{IRSurvey}. 
%Given a question $q$ and a large collection of entity documents $D$, our task can also be viewed as a retrieval problem that involves fetching the correct answer entity $e$ represented by document $d_e \in D$. In contrast to typical adhoc retrieval tasks our questions (queries) are longer and do not have lot of lexical overlap with words in reviews> Thus, models such as BM25 \cite{BM25} are not as effective in ranking candidate answers (See experiments for more details). %We therefore choose to use a neural information retrieval model (IR) such as Duet \cite{DUET} which has been effective on existing QA-style retrieval tasks.  
%In addition, our documents do not have structure in the form of sections and headers that are otherwise useful clues while building retrieval models. However, employing neural models for reading very documents from a large collection as in our task, introduces challenges of scale. Thus in order   Existing QA tasks such as Open-SQuAD \cite{R3} and MS MARCO \cite{MSMARCO} rely on shallow semantic matchers such as those based on BM25 \cite{BM25} ranking to prune the search space before running deeper neural models to re-rank answers on the reduced space. We view  %Since we deal with a large candidate space in our task, typical telescoping architectures that  select-rerank%Due to the large candidate space, using a telescopic ``retrieve-rerank'' architecture that first reduces the search space using quick shallow-semantic and then deeper reasoning  However, in contrast to adhoc retrieval tasks our queries (questions) are much longer and our answering task is not based on factual assertions. Thus, methods such as BM25 \cite{BM25} that are designed for shallow semantic matching do not work well (see experiments for more details). We Neural IR methods such as Duet \cite{DUET} or question-answering methods such as BiDAF \cite{BIDAF} and BERT \cite{BERT} that have multiple layers of cross-attention, are still prohibitively expensive to run for this task. %based on deeper reasoning such as additionally, methods designed for shallow semantic and lexical match   % and requires reasoning over thousands of entity documents. % which are also much larger than existing datasets (See Table \ref{tab:related}). 


%To the best of our knowledge we are the first to propose and attempt such an end-to-end task using a collection of entity reviews.  
%As a first step at attempting this task we create smaller representative documents by clustering sentences for each document in embedding space. This reduces the document size by 70\% and helps improve scalability but we find that commonly used architectures such BiDAF \cite{BIDAF} and BERT \cite{BERT} which have multiple layers of cross-attention are still prohibitively expensive to run for this task. We therefore use a fast and scalable neural method to prune the candidate space for each question and then use a simplified reasoning neural model to rank the final answer. Our model has an Accuracy@3 of $40$\%. % as traditional QA architectures such as those based on BIDAF \cite{BIDAF} and BERT \cite{BERT} do not scale on our task.
 
%We present our first model for this task and formulate the question answering problem as an answer (entity) retrieval and ranking task from a given candidate space of thousands of entities. We use a Siamese network with self-attention (intra-attention) to encode a question and a document consisting of reviews about an entity. The network is trained using a max-margin criterion that aims to score a correct answer (gold answer)\footnote{We use the phrases``gold answer entity'' and ``correct answer entity'' interchangeably in the rest of the paper.} entity higher than an incorrect answer. To make the training of network tractable, we build smaller ``{\em representative documents}'' for each entity.
%The representative documents are created by clustering review sentences in an embedding space \cite{USE2018}. Reviews about an entity tend to be repetitive in the aspects they mention and clustering is a suitable way of balancing diversity and redundancy.
%Sentences from review documents are encoded into a universal sentence embedding space using a pre-trained model \cite{USE2018} and then clustered in embedding space.
%Representative sentences from each cluster constitute the smaller but {\em representative document} for each entity.
%To train the objective function, incorrect answers can be randomly sampled from the candidate space or as our experiments show, better sampling coupled with curriculum learning can improve the model training. Note that, in contrast to most existing tasks where documents are expected to {\em contain} an answer to a question, this task involves reading thousands of documents (each describing an entity), to {\em infer} the best entity answer (document). In effect, this also results in a much weaker signal for supervision as compared to reading comprehension/answer selection tasks, where an explicit answer is marked or identified within a document. %Further, to improve training quality we use curriculum learning and slowly increase . % and provide better negative samples by employing 
%\vspace{-2ex}
%In summary our paper makes the following contributions
%\noindent {\bf Contributions:} [TO BE FIXED] (1) We present the novel task of answering entity-seeking questions using a large collection of entity reviews. Our QA task requires reasoning over thousands of entity documents, where answers to questions in our dataset are different from factual assertions and are {\em subjective}. %Our task also requires reasoning over a much larger collection of documents as compared to existing work. (2) We present models and detailed experiments highlighting the challenges of scale and how a existing methods apply to this task.%which are also much larger than existing datasets %(2) We harvest a novel dataset on tourism questions consisting of $55,514$ QA pairs collected from online travel forums. Each QA pair consists of a question and an answer entity ID, which corresponds to one of the over $200,000$ entity review documents collected from the web. (3)  Gold-answer entities are extracted from mentions in full text user responses to the actual forum post. The entities in our dataset contain 
% Added 'Gold' in point 3 by Aditi - to clarify the difference b/w answer entities in pt 2 & 3
% Hotels, Restaurants 
% Edited to the following by Krunal
%hotels, restaurants
%
%and general attractions of interest in $50$ cities across the world. Answers to questions in our dataset are different from factual assertions and are {\em subjective}. (4) Our QA task requires reasoning over thousands of documents which are also much larger than existing datasets (See Table \ref{tab:related}).  We present the first neural model that scales for this novel task. (5) We present detailed experiments demonstrating the benefits of each of our modeling choices - (a) building representative documents (b) the use of curriculum learning with improved negative sampling. %method that returns better negative samples using a weaker neural model.  %by clustering each sentence in a document in sentence embedding space from a pre-trained model.  siamese architecture We find that existing approaches do not scale for this ask and we devise simple but effective methods 
% Aditi :Shouldn't these points be paired with the points in intro about why our problem is hard
%Since the knowledge source is based on reviews, it can contain conflicting views making the reasoning task harder. %In addition, questions as well as review collections in the knowledge source are noisy in language and are also significantly longer in length than existing datasets. 
% Table \ref{tab:related} compares several attributes of recently released datasets on machine reading at scale and QA with our dataset. 
%    They are also noisy and informal in language.
    

%\section{TourQue QA Task} \label{sec:task}
%Given a large collection of unstructured documents $D$ consisting of a document $d_i$ for each entity $i$ in our dataset, we define the task of answering a question $q$ by returning an an entity $i$.  Each document $d_i$ contains multiple unstructured reviews from real world users along with minimal meta-data such as the entity category, address, rating (where available) etc. Questions are unstructured and have multiple sentences while entity documents can contain thousands of reviews. Our task setting thus, corresponds to a typical information retrieval task where documents (entities described by the documents) can serve as answers to questions (queries).


==> introduction.tex <==
\section{Introduction} \label{sec:introduction}
Recent question answering datasets focus on a variety of tasks such as passage reading comprehension (e.g. SQuAD \cite{SqUAD}, SearchQA \cite{SearchQA}, NewsQA \cite{NewsQA}, TriviaQA \cite{TriviaQA}, HotpotQA \cite{HotpotQA}), Science Question Answering \cite{OpenBookQA2018,ExplanationBank,AI2}, QA using knowledge graphs \cite{WebQuestions,SimpleQuestions,QuizBowl}, Dialog and Sequential QA (e.g. \cite{dinan2018wizard}, QuAC \cite{QuAC}, CoQA \cite{CoQA}, QBLink \cite{QBLink}), Long Form QA \cite{LongFormQA} that requires abstractive or extractive summary answers. Many existing QA tasks that rely on unstructured knowledge are largely formulated as variants of reading comprehension tasks, which assume answers are stated explicitly in the documents \cite{SqUAD,TriviaQA} or require inference over text from one or more passages/articles to generate the exact correct answer \cite{HotpotQA,CoQA,QuAC,LongFormQA}. While these datasets have been useful in furthering research in comprehension, inference and reasoning, we find that they do not always reflect 
% the complex nature of real world information seeking QA. 
% Edited to the following by Krunal
the complexity expressed in real-world question answering.

% Aditi : Can we remove the duplicate use of 'real world' here? 
%
%Real world questions, 
% for instance, 
% Edited to the following by Krunal
%
%such as those seen on online forums are often verbose, requiring us to first determine what is crucial in the question for answering.  Further, answering such questions is also challenging,  as it could also involve reasoning across large unstructured documents.
\begin{figure*}[ht]
 {\footnotesize
 %\begin{adjustwidth}{-2.2cm}{}
 %  Requires \usepackage{graphicx}
 \center
   \includegraphics[scale=0.35]{figs/MSEQ_example.jpg}
   %\vspace*{-2ex}
   \caption{Question from an online travel forum. Figure from \cite{MSEQPaper}}
   \label{fig:queryExample}
 %\end{adjustwidth}
 
 }
% \vspace*{-2.5ex}
 \end{figure*}
For example, consider the question in Figure \ref{fig:queryExample}: Here the user describes {\em who they are}, {\em what they are looking for}, as well as 
% describe their {\em preferences}
% Edited to the following by Krunal
{\em their preferences} for the expected answer.
%
They also mention they are {\em looking forward to the trip} and are going to be {\em first time visitors} to the city. Not all aspects of the question are relevant for answering this query and this makes identifying the informational need challenging. Further, it is worth noting that this question is almost as large as the reading comprehension paragraphs used in tasks such as SQuAD\footnote{Average size of paragraphs in SQuAD is 140 tokens}. %\cite{SqUAD,RetrieveAndReadCIKM}.
% Krunal: Citation problem I think, please check

Answering such questions requires 
% the creation of a real world knowledge 
% Edited to the following by Krunal
understanding knowledge sources which
%
describe possible answer entities in an unstructured or semi-structured form. Knowledge could come from travel articles, blogs, reviews or similar documents.  %A key difference between answering such questions as compared to existing work is that answers are unlikely to be specified explicitly in knowledge. 
%Most existing QA tasks that rely on unstructured knowledge are largely formulated as variants of reading comprehension tasks, which assume answers are stated explicitly in the documents \cite{SqUAD,TriviaQA} or require inference over text from one or more passages/articles to generate the exact correct answer \cite{HotpotQA,CoQA,QuAC}. These assumptions may not hold always in real world. 
Online reviews describing entities of interest can often be informal and noisy, contain subjective opinions, as well as, sentences unrelated to the entity being considered and in some cases, even discuss other entities (e.g., for comparison). %(e.g. when users draw comparisons).
Further, review collections describing entities can be orders of magnitude larger than articles/documents used in %considered large in 
existing QA tasks (see Table \ref{tab:related}) which also brings in challenges associated with scaling unstructured knowledge understanding. Thus, a QA system for this task would need to process thousands of subjective opinion documents (reviews) to
% Aditi : offer a suggestion (entity) 
suggest an entity
as an answer, making the reasoning task harder. %In addition, in contrast to existing tasks where documents contain an answer to a question, this task would involve reading thousands of documents (each describing an entity), to select the best entity answer. Note that this also translates to a weaker signal for supervision as compared to reading comprehension/answer selection tasks, where an explicit answer is marked or identified in a document.  %(See Table \ref{tab:related}). 
% Edited to the following by Krunal
% existing QA models.
%
%(see section \ref{sec:data}).
%\subsection{Contribution}\\


\begin{table*}[]
\scriptsize
\center
\begin{tabular}{c|c|c|c|c|c}
\textbf{Dataset} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Knowledge\\ Source\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Answer \\ type\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg. tokens\\ in documents\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Answer \\ document\\ known\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Multiple docs* \\ required\\ for answering\end{tabular}}}  \\ \hline \hline
\textbf{SQuAD} \cite{SqUAD}        & Wikipedia paragraphs                                                                                         &  Span                                                                                    &  137                                                                                               & Y  & N                                                                                             \\
\textbf{NewsQA}\cite{NewsQA}        & CNN News articles                                                                                        &   Span                                                                                  &  $\approx$ 300                                                                                               & Y  & N                                                                                               \\
\textbf{SearchQA} \cite{SearchQA}       & Web snippets                                                                                        &  Span                                                                                   &  25-46                                                                                               &    N & N                                                                                           \\
\textbf{RACE} \cite{RACE}       & Passages on topics                                                                                        &  Choices                                                                                & 350                                                                                                 & Y               &  N                                                                                \\
\textbf{OpenBookQA} \cite{OpenBookQA2018}       & Fact sentences                                                                                        &  Choices                                                                                &   10                                                                                             & Y               &  Y                                                                                \\
\textbf{MSMARCO} \cite{MSMARCO}       &   Web article snippets                                                                                     &  Free text                                                                                   & 10                                                                                                & N         & Y                                                                                      \\
\textbf{MedQA} \cite{MedQA}        & Medical Articles                                                                                        & Choices                                                                                    &  35                                                                                               & Y              & Y                                                                                 \\
\textbf{WikiReading} \cite{WikiReading}        &  Wikipedia articles                                                                                      & Infobox property                                                                                    &                                                                                         489       &    N                  &    N                                                                       \\
\textbf{TriviaQA} \cite{TriviaQA}        &  Web articles                                                                                       &  Span                                                                                   & 2895$^{\dagger}$                                                                                       & N & Y \\
%\textbf{WikiMovies}        &                                                                                         &                                                                                     &                                                                                                 &                                                                               &                   \\
\textbf{HotPot-QA} \cite{HotpotQA}        & Wikipedia paragraphs                                                                                         & Span                                                                                    &        $\approx$ 300                                                                                         &  N                                                                & Y                               \\
\textbf{ELI5} \cite{LongFormQA}         &  Passages on topics                                                                                       &    Free text                                                                              &                                                                                 858                &     Y                                                                       &    N                \\

\hline
Dialog QA - \textbf{QuAC} \cite{QuAC}         &  Wikipedia passages                                                                                       &    Span                                                                              &                                                                                               401  &     Y                                                                        &    N                \\ 

Dialog QA - \textbf{CoQA} \cite{CoQA}         &  Passages on topics                                                                                       &    Free text                                                                              &                                                                                 271                &     Y                                                                       &    N                \\ 


\textbf{Our Dataset}       &  Reviews                                                                                       & Entity (doc.)                                                                                    &                                                                                  3266 & N & Y %excluding empty entities               & N                                                                             & Y                   \\
\end{tabular}
\caption{Related datasets on Machine reading/QA and their characteristics. In case of Reading comprehension style tasks, the document containing the actual answer may not always be known. * "docs" refers to what the task would consider as its document (eg. Fact sentences in case of OpenBookQA). $^{\dagger}$ Most questions in TriviaQA are answerable using only the first few hundred tokens in the document} %[t TODO:LAST TWO COLUMNS NEED TO BE DOUBLE CHECKED, ADITI TO COMPLETE TABLE]}  
\label{tab:related}
%\vspace{-2.5ex}
\end{table*}

 In this paper, we introduce the novel task of answering entity-seeking recommendation questions using a collection of reviews describing entities. Our work is inspired by  \citeauthor{MSEQPaper}'s recent work on parsing and understanding multi-sentence entity seeking questions. Their work does not attempt to solve a QA task end-to-end and relies on a pipeline consisting of semantic parsing and the availability of a Web API to try and answer such questions. For this task we harvest a novel dataset on tourism questions consisting of $48,147$ QA pairs collected from online travel forums. Each QA pair consists of a question and an answer entity ID, which corresponds to one of the over $200,000$ entity review documents collected from the web. Gold-answer entities are extracted from mentions in full text user responses to the actual forum post. The entities in our dataset contain 
% Added 'Gold' in point 3 by Aditi - to clarify the difference b/w answer entities in pt 2 & 3
% Hotels, Restaurants 
% Edited to the following by Krunal
hotels, restaurants
%
and general attractions of interest in $50$ cities across the world. Answers to questions in our dataset are different from factual assertions and are {\em subjective}. % and requires reasoning over thousands of entity documents. % which are also much larger than existing datasets (See Table \ref{tab:related}). 


To the best of our knowledge we are the first to propose and attempt such an end-to-end task using a collection of entity reviews.  As a first step at attempting this task we create smaller representative documents by clustering sentences for each document in embedding space. This reduces the document size by 70\% and helps improve scalability but we find that commonly used architectures such BiDAF \cite{BIDAF} and BERT \cite{BERT} which have multiple layers of cross-attention are still prohibitively expensive to run for this task. We therefore use a fast and scalable neural method to prune the candidate space for each question and then use a simplified reasoning neural model to rank the final answer. Our model has an Accuracy@3 of $40$\%. % as traditional QA architectures such as those based on BIDAF \cite{BIDAF} and BERT \cite{BERT} do not scale on our task.
 
%We present our first model for this task and formulate the question answering problem as an answer (entity) retrieval and ranking task from a given candidate space of thousands of entities. We use a Siamese network with self-attention (intra-attention) to encode a question and a document consisting of reviews about an entity. The network is trained using a max-margin criterion that aims to score a correct answer (gold answer)\footnote{We use the phrases``gold answer entity'' and ``correct answer entity'' interchangeably in the rest of the paper.} entity higher than an incorrect answer. To make the training of network tractable, we build smaller ``{\em representative documents}'' for each entity.
%The representative documents are created by clustering review sentences in an embedding space \cite{USE2018}. Reviews about an entity tend to be repetitive in the aspects they mention and clustering is a suitable way of balancing diversity and redundancy.
%Sentences from review documents are encoded into a universal sentence embedding space using a pre-trained model \cite{USE2018} and then clustered in embedding space.
%Representative sentences from each cluster constitute the smaller but {\em representative document} for each entity.
%To train the objective function, incorrect answers can be randomly sampled from the candidate space or as our experiments show, better sampling coupled with curriculum learning can improve the model training. Note that, in contrast to most existing tasks where documents are expected to {\em contain} an answer to a question, this task involves reading thousands of documents (each describing an entity), to {\em infer} the best entity answer (document). In effect, this also results in a much weaker signal for supervision as compared to reading comprehension/answer selection tasks, where an explicit answer is marked or identified within a document. %Further, to improve training quality we use curriculum learning and slowly increase . % and provide better negative samples by employing 
%\vspace{-2ex}
%In summary our paper makes the following contributions
\noindent {\bf Contributions:} [TO BE FIXED] (1) We present the novel task of answering entity-seeking questions using a large collection of entity reviews. Our QA task requires reasoning over thousands of entity documents, where answers to questions in our dataset are different from factual assertions and are {\em subjective}. %Our task also requires reasoning over a much larger collection of documents as compared to existing work.
(2) We present models and detailed experiments highlighting the challenges of scale and how existing methods apply to this task.%which are also much larger than existing datasets %(2) We harvest a novel dataset on tourism questions consisting of $55,514$ QA pairs collected from online travel forums. Each QA pair consists of a question and an answer entity ID, which corresponds to one of the over $200,000$ entity review documents collected from the web. (3)  Gold-answer entities are extracted from mentions in full text user responses to the actual forum post. The entities in our dataset contain 
% Added 'Gold' in point 3 by Aditi - to clarify the difference b/w answer entities in pt 2 & 3
% Hotels, Restaurants 
% Edited to the following by Krunal
%hotels, restaurants
%
%and general attractions of interest in $50$ cities across the world. Answers to questions in our dataset are different from factual assertions and are {\em subjective}. (4) Our QA task requires reasoning over thousands of documents which are also much larger than existing datasets (See Table \ref{tab:related}).  We present the first neural model that scales for this novel task. (5) We present detailed experiments demonstrating the benefits of each of our modeling choices - (a) building representative documents (b) the use of curriculum learning with improved negative sampling. %method that returns better negative samples using a weaker neural model.  %by clustering each sentence in a document in sentence embedding space from a pre-trained model.  siamese architecture We find that existing approaches do not scale for this ask and we devise simple but effective methods 
% Aditi :Shouldn't these points be paired with the points in intro about why our problem is hard
%Since the knowledge source is based on reviews, it can contain conflicting views making the reasoning task harder. %In addition, questions as well as review collections in the knowledge source are noisy in language and are also significantly longer in length than existing datasets. 
% Table \ref{tab:related} compares several attributes of recently released datasets on machine reading at scale and QA with our dataset. 
%    They are also noisy and informal in language.
    

%\section{TourQue QA Task} \label{sec:task}
%Given a large collection of unstructured documents $D$ consisting of a document $d_i$ for each entity $i$ in our dataset, we define the task of answering a question $q$ by returning an an entity $i$.  Each document $d_i$ contains multiple unstructured reviews from real world users along with minimal meta-data such as the entity category, address, rating (where available) etc. Questions are unstructured and have multiple sentences while entity documents can contain thousands of reviews. Our task setting thus, corresponds to a typical information retrieval task where documents (entities described by the documents) can serve as answers to questions (queries).


==> task_def.tex <==
% \section{Task Definition}
% Given an entity seeking recommendation question ($q$), its target class ($t \in $ \{hotel, attraction, restaurant\}), the city $c$, a candidate space of entities $E_c^t$ for each corresponding city and entity class, a collection of their reviews $R_c^t$; the goal of this task is to find the correct (gold) answer entity $a \in E_c^t$ using the documents $R_c^t$ describing the candidate answer entities.

\section{Task Definition} \label{sec:data}
%\section{Task Definition}
Given an entity seeking recommendation question ($q$), its target class ($t \in $ \{hotel, attraction, restaurant\}), the city $c$, a candidate space of entities $E_c^t$ for each corresponding city and entity class, a collection of their reviews $R_c^t$; the goal of this task is to find the correct (gold) answer entity $a \in E_c^t$ using the documents $R_c^t$ describing the candidate answer entities.

